Membership Inference Attacks and Defenses in Neural Network Pruning

Neural network pruning has been an essential technique to reduce the computation and memory requirements for using deep neural networks for resource-constrained devices. Most existing research focuses primarily on balancing the sparsity and accuracy of a pruned neural network by strategically removing insignificant parameters and retraining the pruned model. Such efforts on reusing training samples pose serious privacy risks due to increased memorization, which, however, has not been investigated yet. In this paper, we conduct the first analysis of privacy risks in neural network pruning. Specifically, we investigate the impacts of neural network pruning on training data privacy, i.e., membership inference attacks. We first explore the impact of neural network pruning on prediction divergence, where the pruning process disproportionately affects the pruned model's behavior for members and non-members. Meanwhile, the influence of divergence even varies among different classes in a fine-grained manner. Enlighten by such divergence, we proposed a self-attention membership inference attack against the pruned neural networks. Extensive experiments are conducted to rigorously evaluate the privacy impacts of different pruning approaches, sparsity levels, and adversary knowledge. The proposed attack shows the higher attack performance on the pruned models when compared with eight existing membership inference attacks. In addition, we propose a new defense mechanism to protect the pruning process by mitigating the prediction divergence based on KL-divergence distance, whose effectiveness has been experimentally demonstrated to effectively mitigate the privacy risks while maintaining the sparsity and accuracy of the pruned models.

==> backup.tex <==
\begin{figure}[!t]
    \centering
    \includegraphics[width=\linewidth]{figs/pipeline.png}
    \caption{\textbf{The workflow of neural network pruning}.}
    \label{fig:pipeline}
\end{figure}


\subsection{Neural Network Pruning Workflow} %
This paper is focused on a general neural network pruning process, whose workflow includes three key stages: original network training, coarse pruning, and fine-tuning, as illustrated in Figure~\ref{fig:pipeline}. Specifically,
\begin{enumerate}
\item \textit{Original network training}: Train a large (sometimes over-parameterized) model $f(\bm{x}; \bm{W})$ with parameters $\bm{W}$;
\vspace{-0.5em}
\item \textit{Coarse pruning}: Prune the trained model by removing the parameters according to a certain criterion. Pruning takes $f(\bm{x}; \bm{W})$ as input and produces a new model $f(\bm{x}; \bm{M}\odot \bm{W})$, where $\bm{M}\in {0, 1}^{|\bm{W}|}$ denotes the binary mask that sets certain parameters to 0, and $\odot$ denotes the element-wise multiplication; 
\vspace{-0.5em}
\item \textit{Fine-tuning}: Fine-tune the pruned model by retraining it on the same training data for $N$ epochs. After fine-tuning, we get the pruned model $f(\bm{x}; \bm{M}\odot \bm{W}')$ with a new set of parameters $\bm{W}'$ different from $\bm{W}$. For simplicity's sake, in the following paper, we use $f$ to denote the original model $f(\bm{x}; \bm{W})$ and $f_p$ to denote the pruned model $f(\bm{x}; M\odot \bm{W}')$. 
\end{enumerate}


\subsection{Adversarial Knowledge}
The goal of a membership inference attack is to determine the membership information given a data sample, \ie, whether the data sample is used to train the target pruned model or not.  
We assume the adversary has the following knowledge:
\begin{itemize}
\item The adversary has access to the target pruned model. The adversary has no access to the original model, which is practical in most real-world cases: the original model for training is not exposed to the public. Only the target pruned model in production is released for public use. 
\vspace{-0.5em}
\item The adversary has access to prediction vector provided by the target pruned model, which means we consider the black-box membership inference attacks, where the internal information about the target pruned model (\eg, the activations in the model) and all the information related to the original model are inaccessible to the adversary.  Compared with white-box attacks (\eg, \cite{nasr2019comprehensive}), the black-box setting is more serious since it can be conducted by anyone who can query the target pruned model.
\vspace{-0.5em}
\item The adversary knows the approaches used for neural network pruning. The adversary can train a shadow model using the same pruning approach. 
\end{itemize}


\subsection{Adaptive Adversary}
The arms race between attacks and defenses is one of the main challenges in machine learning privacy. 
If the defense is designed without considering the adversary knows the defense mechanisms, usually the defense performance will be substantially degraded after the adaptive attacks are evaluated against the defense. 
Hence, it is critical to consider both non-adaptive and adaptive attacks in evaluating the defense mechanisms.
In this paper, we consider two types of attacks: 1) non-adaptive attacks - the adversary does not know the defense mechanism and trains the shadow pruned model only using neural network pruning; 2) adaptive attacks - the adversary knows the defense mechanism and trains the shadow pruned model using neural network pruning with the same defense.


\subsection{Neural Network Pruning}
The state-of-the-art neural networks are usually deep and resource hungry, requiring large amounts of computation and memory, which becomes a particular challenge on resource-constrained end devices. As one of the most popular network compression approach, neural network pruning has attracted great attention in recent years~\cite{mozer1989skeletonization,janowsky1989pruning,segee1991fault,reed1993pruning}. 
Train-Prune-Fine-tuning is the most common way to achieve the good performance of the pruned models. In this paper, we evaluate the privacy risk of pruned models following this setting. Recently, alternative approaches such as rewinding the pruned model's weight values to an earlier state~\cite{frankle2018lottery} and fine-tuning the pruned model using the original training schedule~\cite{renda2020comparing} are shown comparable performance with the original model. We will investigate the privacy risks of these pruning approaches in our future work.
To prune the parameters in the neural networks, recently Han \etal proposed to remove the parameters with the lowest absolute values~\cite{han2015deep}. To facilitate hardware optimization and accelerate the neural network computation, many methods were proposed to remove parameters in an organized way (structured pruning) by removing the entire filters or channels~\cite{li2016pruning,liu2017learning}. 


Although most studies on network pruning focus on the overall accuracy of pruned models on test data, some efforts have been put into the other effects caused by network pruning.
Paganini~\cite{paganini2020prune} investigated the unfairness and systematic biases in the pruned models. Hooker \etal~\cite{hooker2019compressed} demonstrated the biased performance on different groups and classes after pruning. 
In this work, we investigate another urgent aspect in network pruning - training data privacy. This work investigates four widely used pruning approaches, including the structured and unstructured approaches, and evaluates the privacy risk of models after pruning.



\subsection{Membership Inference Attacks}
Given a target machine learning model $f: \mathbb{R}^n \rightarrow \mathbb{R}$, the goal of membership inference attacks is to infer whether a given data sample was used in the model training or not. 
Formally, membership inference attack can be defined as:
\begin{equation}
    \mathcal{A}: \bm{x}, f \rightarrow \{0, 1\},
\end{equation}
where $\mathcal{A}$ denotes the attack model, which is a binary classifier. If the data sample $\bm{x}$ is used to train the target model $f$ , $\mathcal{A}$ outputs $1$ (\ie, member), and $0$ otherwise (\ie, non-member).

In this paper, we consider the black-box setting of membership inference attacks, where the adversary only has access to the target model's prediction given a data sample. 
For example, Shokri~\etal~\cite{shokri2015privacy} constructed several shadow models to mimic the target model's different behaviors on the predictions of members and non-members and then train a binary classifier based on the predictions as an attack model to determine the membership of data samples against the target model. Salem~\etal~\cite{salem2018ml} found that membership inference attacks are successful even using a single shadow model. Nasr~\etal~\cite{nasr2018machine} added the class labels of data samples to the input of the attack model to improve the attack accuracy. 
In addition to the neural network-based attack models, Leino~\etal~\cite{leino2020stolen}, Yeom~\etal~\cite{yeom2018privacy}, and Song~\etal~\cite{song2019privacy,song2020systematic} found that some metrics derived from model predictions can be used as a sign of membership. The metric-based attacks determine a given data sample is a member if the metric of this given sample (\eg, confidence, entropy, modified entropy) is above a certain threshold.  
Song~\etal recently showed that by setting class-dependent threshold, the metric-based attacks could achieve comparable or even better performance compared with neural network-based attacks.
Hence, in this paper, we use two metric-based attacks proposed in~\cite{song2020systematic} as our baseline attacks.
Besides, most neural network-based attack models were built upon fully-connected neural networks, which might not thoroughly explore the connections between predictions and labels. In this paper, we propose a self-attention-based membership inference attack to leverage the dependence of input features such as model predictions and sample labels. Our evaluation results demonstrate the superior performance of our proposed self-attention-based attack.


\subsection{Defenses against Membership Inference Attacks}
Several defenses against membership inference attacks have been proposed to mitigate privacy risks in machine learning models. 
Differential privacy (DP)~\cite{dwork2008differential,dwork2006calibrating,abadi2016deep} is a widely used privacy-preserving technique to provide provable privacy risk mitigation by adding noise to the gradient or parameters during training. 
However, DP requires a large magnitude of noises to achieve a meaningful theoretical privacy guarantee, which significantly degrades the performance of the protected models~\cite{jayaraman2019evaluating}. 
Regularization~\cite{shokri2017membership}, dropout, and model stacking were used \etal~\cite{salem2019ml} in target model training to reduce privacy risks by avoiding overfitting. Although these approaches reduced the vulnerability by bridging the generalization gap between member and non-member data, in many cases, the privacy risks after applying these approaches are still high.
Nasr~\etal~\cite{nasr2018machine} trained the target model with additional adversarial regularization to defend against membership inference attacks. 
Jia~\etal~\cite{jia2019memguard} conducted adversarial attacks~\cite{yuan2019adversarial} against the adversary's attack model by intentionally modifying the target model's predictions to mislead the attack model.
According to the recent analysis of defenses against membership inference attacks, most of these defenses are either limited in the effectiveness against adaptive attacks~\cite{niu2020membership,song2020systematic} or no better than the early stopping mechanisms~\cite{song2020systematic}. 
Therefore, in this paper, we use the early stopping mechanism as our baseline defense. We evaluate the performance of our proposed defense with both non-adaptive and adaptive attacks.



In this section, we first provide some insights on why neural network pruning makes the model more vulnerable to membership inference attacks and then describe the general membership inference attacks against neural network pruning. We introduce two types of membership inference attacks to evaluate the privacy risks of pruned models. 

\newsavebox{\measurebox}

\begin{figure*}[!t]
\centering
\sbox{\measurebox}{%
\begin{minipage}[b]{.4\textwidth}
\begin{subfigure}[b]{\textwidth}
\includegraphics[width=0.9\textwidth]{figs/cifar100_mobilenetv2_avg_div.png}
\caption{CIFAR100 dataset}
\end{subfigure}
\end{minipage}}
\usebox{\measurebox}\qquad
\begin{minipage}[b][\ht\measurebox][s]{.4\textwidth}
\centering
\begin{subfigure}[b]{\textwidth}
\includegraphics[width=0.9\textwidth]{figs/cifar10_mobilenetv2_avg_div.png}
\caption{CIFAR10 dataset}
\end{subfigure}

\begin{subfigure}[b]{\textwidth}
\vspace{0.2cm}
\hspace{0.7cm}
\includegraphics[width=0.8\textwidth]{figs/svhn_mobilenetv2_avg_div.png}
\caption{SVHN dataset}
\end{subfigure}
\end{minipage}
\caption{\textbf{Divergence of the Pruned Model's Prediction Confidences over Different Classes.} We prune three MobileNetV2 models with 70\% sparsity on the CIFAR100, CIFAR10, and SVHN datasets, respectively. The red bar indicates the average prediction confidence of members in each class. The green bar indicates the average prediction confidence of non-members. We observe that the divergence of predictions between members and non-members (difference of average prediction confidence between members and non-members, shown in the blue curve) differ among classes. For example, for the CIFAR100 dataset, the divergence in the class ``fox'' is around three times higher than that in the class ``cloud''. (We only show the first 40 classes in the CIFAR100 dataset due to space limit.)}
\label{fig:cls_div}
\end{figure*}

\subsection{Divergence of Prediction Confidences}
Although neural network pruning helps remove the redundant parameters, recent research on neural network pruning usually focuses on improving the trade-off between the pruned models' sparsity and their overall prediction performance (\ie, test accuracy). 
However, we observe that despite the overall prediction performance is not degraded, neural network pruning may disproportionately affect the pruned models' prediction performance on the training data (members) and test data (non-members). Such disproportionate effects might increase the divergence between predictions over members and non-members (Figure~\ref{fig:histogram}).
Given that most existing membership inference attacks predict the membership status based on the difference of predictions between members and non-members, such increased divergence in neural network pruning makes the pruned models more vulnerable to membership inference attacks.

More importantly, we observe that the disproportionate effects of neural network pruning vary widely among the different subgroups of training and test data. 
Figure~\ref{fig:cls_div} shows that the divergence of the pruned models' predictions over members and non-members is significantly different among classes.
Moreover, the divergence may differ greatly among the subgroups of each class, where the divergence of predictions over subgroups of each class can be affected by neural network pruning in different degrees.
Similar observation of divergence on different subgroups after neural network pruning has been made in other fields such as model fairness and transparency~\cite{paganini2020prune,hooker2019compressed,hooker2020characterising}.
We hypothesize that such divergence among subgroups may provide fine-grained ``evidence'' for membership inference attacks and lead to more serious privacy leakage.

Therefore, in the following sections, we investigated the pruned models' privacy risks by analyzing divergence of prediction confidences over members and non-members and among different classes.

\begin{figure}[!t]
    \centering
    \includegraphics[width=0.95\linewidth]{figs/attack_pipeline.png}
    \caption{{The framework of membership inference attacks (MIA) against neural network pruning.}}
    \label{fig:attack_pipeline}
\end{figure}

\subsection{Proposed Attack Design against Neural Network Pruning}
To explore the performance divergence due to neural network pruning, 
we adopt the shadow model training strategy in general attack design by training both the shadow model and shadow pruned model.
The shadow pruned model provides the evidence how neural network pruning changes the predictions for each subgroup.
Shadow model training strategy is widely used in most membership inference attacks. 

In our proposed membership inference attacks, the adversary first trains a shadow model from shadow member data (\ie, training data used in the shadow model), and then prunes and fine-tunes the shadow model using the same neural network pruning approach. 
Based on the predictions of the shadow pruned model, the adversary trains an attack model to learn how to distinguish shadow member data and shadow non-member data.
To extract sensitive membership information from the target pruned model, the adversary first derives the predictions of the given input sample by querying the target pruned model. The the adversary feeds the predictions into the trained attack model and provides the binary classification of the membership status.
Figure~\ref{fig:attack_pipeline} illustrates the general design of membership inference attacks against neural network pruning.

Next, we introduce two types of membership inference attacks to explore the privacy risks in neural network pruning.

\subsection{Class Dependent MIA} %
Inspired by recent threshold-based membership inference attacks~\cite{leino2020stolen,yeom2018privacy,song2020systematic}, we introduce class-dependent threshold-based attacks to infer the membership of the data samples. The adversary learns the thresholds from the shadow pruned model according to different class-dependent metrics (\eg, prediction confidence, correctness, and entropy). The adversary predicts an input sample is a member if the metric is above the threshold, and vice versa. 
Specifically, we select two metrics for class-dependent threshold-based attacks: prediction confidence and modified entropy. Yeom \etal, used prediction confidence to identify membership status of an input sample~\cite{yeom2018privacy}. Song \etal, recently proposed modified entropy, which achieved better performance than using prediction confidence~\cite{song2020systematic}.

Given an input sample $\bm{x}$, its class $y$ and target pruned model $f_p$, the class-dependent threshold-based attack using prediction confidence (``conf'' attack for short) is defined as follows:
\begin{equation}
    I_{\mathrm{conf}}(f_p, (\bm{x},y)) = \mathbbm{1}\{f_p^{(y)}(\bm{x})\geq\zeta_y\},
\end{equation}
where $f^{(y)}$ denotes the prediction confidence of class $y$ and $\zeta_y$ is the threshold of class $y$ derived from the shadow pruned model. $\mathbbm{1}{}$ denotes the indicator, which outputs $1$ (\ie, member) if the prediction confidence is larger than the threshold in class $y$, $0$ (\ie, non-member) otherwise. Similarly, we define the class dependent threshold-based attack using another metric, modified entropy (``mentr'' attack for short) as follows:
\begin{equation}
    I_{\mathrm{mentr}}(f_p, (\bm{x},y)) = \mathbbm{1}\{\mathrm{mentr}(f_p^{(y)}(\bm{x}))\geq\zeta_y\},
\end{equation}
where modified entropy is defined as:
\begin{align}
\mathrm{mentr}(f_p(\bm{x}), y) =& - (1 - f_p^{(y)}(\bm{x}))\log (f_p^{(y)}(\bm{x})) \nonumber\\
&- \sum_{t\neq y}f_p^{(t)}(\bm{x})\log(1-f_p^{(t)}(\bm{x})).
\end{align}

By extracting the class dependent thresholds according to these two metrics, the adversary is capable of identifying the fine-grained divergence between members and non-members. 
The adversary infers an input sample is a member if the metric is above the class-dependent threshold, and non-member otherwise. 
The implementation of our class dependent threshold-based attacks is adapt from Song \etal's work\footnote{\url{https://github.com/inspire-group/membership-inference-evaluation}}.
Our evaluation showed that class-dependent threshold-based attacks explore more serious privacy risks of the pruned models than those of the original models.

\subsection{Self-Attention MIA (SAMIA)} %
\begin{figure}[!t]
    \centering
    \includegraphics[width=\linewidth]{figs/self-attention.png}
    \caption{Network Architecture for Self-Attention-based Membership Inference Attack.}
    \label{fig:self_attention}
\end{figure}
The class dependent threshold-based membership inference attacks may underestimate the privacy risks due to neural network pruning since the divergence of predictions disproportionately affects not only the different classes but also specific subgroups of data samples. 
A single threshold for a class may not represent the different degrees of the divergence of predictions among subgroups.

To conduct finer-grained analysis of divergence among subgroups, we propose a self-attention-based membership inference attack (SAMIA). Self-attention is an essential component to capture global dependencies and is widely used in the state-of-the-art natural language processing models such as GPT3~\cite{brown2020language}, BERT~\cite{devlin2019bert,vaswani2017attention}. 
Despite the recent advances, the self-attention mechanism has not yet been included in the research of privacy attacks. 

In SAMIA, we leverage the self-attention mechanism to automatically extract the finer-grained ``thresholds'' from different classes and subgroups by capturing the dependency between predictions and label classes using neural networks. 
SAMIA takes the pruned model's predictions and ground-truth labels as inputs.  
The self-attention mechanism constructs subgroups based on model predictions and labels automatically and, moreover, finds out which subgroup the attack ``threshold'' should pay more ``attention.'' 
The outputs of the self-attention mechanism will be the weighted sum of the inputs over the attention scores.
By applying self-attention mechanism, SAMIA derives more finer-grained ``thresholds'' in terms of subgroups than the class dependent thresholds. 
Our evaluation demonstrates that SAMIA leads to higher attack accuracy compared with two threshold-based attacks.

Figure~\ref{fig:self_attention} illustrates the network architecture of the attack model used in SAMIA. We first convert the ground-truth label into a one-hot label and then feed both the pruned model's prediction and one-hot label into the attack model as the input features. 
The input features are first encoded into a vector using a Fully Connected (FC) layer to form subgroups and then transformed as query $Q$, key $K$, and value $V$ vectors using a linear function.
The attention module calculates the attention scores of the subgroups in a scaled dot-product way:
\begin{equation}
    \mathrm{Attention}(Q, K, V) = \mathrm{softmax}(QK^T)V,
\end{equation}
where $\mathrm{softmax}()$ denotes the softmax function to make the attention scores sum up to $1$.
The output of the attention module is the weighted sum of the value vector, where the weight assigned to each value is derived by the attention scores $\mathrm{softmax}(QK^T)$. 
Followed by the attention module, we apply dropout to the output of the attention module to avoid overfitting and create a shortcut (residual) connection between the input and output of the attention module to avoid gradient vanishing. 
In the attack model of SAMIA, we adopt two attention modules, followed by two fully connected layers. 
A non-linear activation function, LeakyReLU~\cite{maas2013rectifier} is applied to the first and fourth FC layers in Figure~\ref{fig:self_attention}. 
We use softmax to provide the binary prediction on the membership. 

Given the workflow of neural network pruning presented in Section~\ref{S3.1}, this section investigates the privacy risks of pruning. A general framework of the membership inference attacks against the pruned model is illustrated in Figure~\ref{fig:attack_pipeline}. 

To extract sensitive membership information from the target pruned model, the adversary first derives the predictions of the given input sample by querying the target pruned model. The the adversary feeds the predictions into the trained attack model and provides the binary classification of the membership status.


\begin{figure}[!t]
    \centering
    \includegraphics[width=0.95\linewidth]{figs/attack_pipeline.png}
    \caption{The framework of membership inference attacks (MIA) against neural network pruning. \todo{sample pool}}
    \label{fig:attack_pipeline}
\end{figure}


\newsavebox{\measurebox}

\begin{figure*}[!t]
\centering
\sbox{\measurebox}{%
\begin{minipage}[b]{.48\textwidth}
\begin{subfigure}[b]{\textwidth}
\includegraphics[width=1.0\textwidth]{figs/cifar100_mobilenetv2_avg_div.png}
\caption{CIFAR100 dataset}
\end{subfigure}
\end{minipage}}
\usebox{\measurebox}\qquad
\begin{minipage}[b][\ht\measurebox][s]{.48\textwidth}
\centering
\begin{subfigure}[b]{\textwidth}
\hspace{4.5cm}
\includegraphics[width=0.3\textwidth]{figs/avg_div_legend.png}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}
\includegraphics[width=0.9\textwidth]{figs/cifar10_mobilenetv2_avg_div.png}
\caption{CIFAR10 dataset}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}
\hspace{1.0cm}
\includegraphics[width=0.8\textwidth]{figs/svhn_mobilenetv2_avg_div.png}
\caption{SVHN dataset}
\end{subfigure}
\end{minipage}
\caption{\textbf{Divergence of the Pruned Model's Prediction Confidences over Different Classes.} We prune three MobileNetV2 models with 70\% sparsity on the CIFAR100, CIFAR10, and SVHN datasets, respectively. The red bar indicates the average prediction confidence of members in each class. The green bar indicates the average prediction confidence of non-members. We observe that the divergence of predictions between members and non-members (difference of average prediction confidence between members and non-members, shown in the blue curve) differ among classes. For example, for the CIFAR100 dataset, the divergence in the class ``fox'' is around three times higher than that in the class ``cloud''. (We only show the first 40 classes in the CIFAR100 dataset due to space limit.)}
\label{fig:cls_div}
\end{figure*}

\subsection{Divergence of Prediction Confidences}
Although neural network pruning helps remove the redundant parameters, recent research on neural network pruning usually focuses on improving the trade-off between the pruned models' sparsity and their overall prediction performance (\ie, test accuracy). 
However, we observe that despite the overall prediction performance is not degraded, neural network pruning may disproportionately affect the pruned models' prediction performance on the training data (members) and test data (non-members). Such disproportionate effects might increase the divergence between predictions over members and non-members (Figure~\ref{fig:histogram}).
Given that most existing membership inference attacks predict the membership status based on the difference of predictions between members and non-members, such increased divergence in neural network pruning makes the pruned models more vulnerable to membership inference attacks.

More importantly, we observe that the disproportionate effects of neural network pruning vary widely among the different subgroups of training and test data. 
Figure~\ref{fig:cls_div} shows that the divergence of the pruned models' predictions over members and non-members is significantly different among classes.
Moreover, the divergence may differ greatly among the subgroups of each class, where the divergence of predictions over subgroups of each class can be affected by neural network pruning in different degrees.
Similar observation of divergence on different subgroups after neural network pruning has been made in other fields such as model fairness and transparency~\cite{paganini2020prune,hooker2019compressed,hooker2020characterising}.
We hypothesize that such divergence among subgroups may provide fine-grained ``evidence'' for membership inference attacks and lead to more serious privacy leakage.
Therefore, in the following sections, we investigated the pruned models' privacy risks by analyzing divergence of prediction confidences over members and non-members and among different classes.
Next, we introduce two types of membership inference attacks to explore the privacy risks in neural network pruning.



\subsection{CDMIA: Class-Dependent MIA} %
Inspired by recent threshold-based membership inference attacks~\cite{leino2020stolen,yeom2018privacy,song2020systematic}, we introduce class-dependent threshold-based attacks to infer the membership of the data samples. The adversary learns the thresholds from the shadow pruned model according to different class-dependent metrics (\eg, prediction confidence, correctness, and entropy). The adversary predicts an input sample is a member if the metric is above the threshold, and vice versa. 
Specifically, we select two metrics for class-dependent threshold-based attacks: prediction confidence and modified entropy. Yeom \etal, used prediction confidence to identify membership status of an input sample~\cite{yeom2018privacy}. Song \etal, recently proposed modified entropy, which achieved better performance than using prediction confidence~\cite{song2020systematic}.

Given an input sample $\bm{x}$, its class $y$ and target pruned model $f_p$, the class-dependent threshold-based attack using prediction confidence (``conf'' attack for short) is defined as follows:
\begin{equation}
    I_{\mathrm{conf}}(f_p, (\bm{x},y)) = \mathbbm{1}\{f_p^{(y)}(\bm{x})\geq\zeta_y\},
\end{equation}
where $f^{(y)}$ denotes the prediction confidence of class $y$ and $\zeta_y$ is the threshold of class $y$ derived from the shadow pruned model. $\mathbbm{1}{}$ denotes the indicator, which outputs $1$ (\ie, member) if the prediction confidence is larger than the threshold in class $y$, $0$ (\ie, non-member) otherwise. Similarly, we define the class dependent threshold-based attack using another metric, modified entropy (``mentr'' attack for short) as follows:
\begin{equation}
    I_{\mathrm{mentr}}(f_p, (\bm{x},y)) = \mathbbm{1}\{\mathrm{mentr}(f_p^{(y)}(\bm{x}))\geq\zeta_y\},
\end{equation}
where modified entropy is defined as:
\begin{align}
\mathrm{mentr}(f_p(\bm{x}), y) =& - (1 - f_p^{(y)}(\bm{x}))\log (f_p^{(y)}(\bm{x})) \nonumber\\
&- \sum_{t\neq y}f_p^{(t)}(\bm{x})\log(1-f_p^{(t)}(\bm{x})).
\end{align}

By extracting the class dependent thresholds according to these two metrics, the adversary is capable of identifying the fine-grained divergence between members and non-members. 
The adversary infers an input sample is a member if the metric is above the class-dependent threshold, and non-member otherwise. 
The implementation of our class dependent threshold-based attacks is adapt from Song \etal's work\footnote{\url{https://github.com/inspire-group/membership-inference-evaluation}}.
Our evaluation showed that class-dependent threshold-based attacks explore more serious privacy risks of the pruned models than those of the original models.


\begin{figure}[!t]
    \centering
    \includegraphics[width=\linewidth]{figs/self-attention.png}
    \caption{The network architecture of the proposed  SAMIA.}
    \label{fig:self_attention}
\end{figure}
\subsection{SAMIA: Self-Attention MIA} %
The CDMIA may underestimate the privacy risks of the pruned neural network since the divergence of predictions disproportionately affects not only the different classes but also specific subgroups of data samples. 
A single threshold for a class may not represent the different degrees of the divergence of predictions among subgroups.

To conduct finer-grained analysis of divergence among subgroups, we propose a self-attention-based membership inference attack (SAMIA). Self-attention is an essential component to capture global dependencies and is widely used in the state-of-the-art natural language processing models such as GPT3~\cite{brown2020language}, BERT~\cite{devlin2019bert,vaswani2017attention}. 
Despite the recent advances, the self-attention mechanism has not yet been included in the research of privacy attacks. 

In SAMIA, we leverage the self-attention mechanism to automatically extract the finer-grained ``thresholds'' from different classes and subgroups by capturing the dependency between predictions and label classes using neural networks. 
SAMIA takes the pruned model's predictions and ground-truth labels as inputs.  
The self-attention mechanism constructs subgroups based on model predictions and labels automatically and, moreover, finds out which subgroup the attack ``threshold'' should pay more ``attention.'' 
The outputs of the self-attention mechanism will be the weighted sum of the inputs over the attention scores.
By applying self-attention mechanism, SAMIA derives more finer-grained ``thresholds'' in terms of subgroups than the class dependent thresholds. 
Our evaluation demonstrates that SAMIA leads to higher attack accuracy compared with two threshold-based attacks.

Figure~\ref{fig:self_attention} illustrates the network architecture of the attack model used in SAMIA. We first convert the ground-truth label into a one-hot label and then feed both the pruned model's prediction and one-hot label into the attack model as the input features. 
The input features are first encoded into a vector using a Fully Connected (FC) layer to form subgroups and then transformed as query $Q$, key $K$, and value $V$ vectors using a linear function.
The attention module calculates the attention scores of the subgroups in a scaled dot-product way:
\begin{equation}
    \mathrm{Attention}(Q, K, V) = \mathrm{softmax}(QK^T)V,
\end{equation}
where $\mathrm{softmax}()$ denotes the softmax function to make the attention scores sum up to $1$.
The output of the attention module is the weighted sum of the value vector, where the weight assigned to each value is derived by the attention scores $\mathrm{softmax}(QK^T)$. 
Followed by the attention module, we apply dropout to the output of the attention module to avoid overfitting and create a shortcut (residual) connection between the input and output of the attention module to avoid gradient vanishing. 
In the attack model of SAMIA, we adopt two attention modules, followed by two fully connected layers. 
A non-linear activation function, LeakyReLU~\cite{maas2013rectifier} is applied to the first and fourth FC layers in Figure~\ref{fig:self_attention}. 
We use softmax to provide the binary prediction on the membership. 

Much of the progress in artificial intelligence over the past decade has been the result of deep neural networks. These powerful neural networks with a large number of parameters consume considerable storage and memory bandwidth. This makes it challenging to deploy the state-of-the-art neural networks on resource-constrained devices. To address this issue, neural network pruning as one of the most popular compression technologies has attracted great attention~\cite{mozer1989skeletonization,han2015deep}. By removing weak connections from a deep neural network, recent research has shown that neural network pruning can substantially reduce the size of a neural network without largely compromising prediction accuracy~\cite{han2015deep,li2016pruning,liu2017learning,blalock2020state}. 

In general, neural network pruning includes three main stages: 1) train an original deep neural network (sometimes over-parameterized); 2) remove the insignificant parameters; 3) fine-tune the remaining parameters with the training dataset so as to reach the expected performance~\cite{blalock2020state}. Most existing research on neural network pruning has focused on improving the trade-off between accuracy and sparsity by strategically design the last two stages~\cite{han2015deep,li2016pruning,liu2017learning,blalock2020state}. However, such efforts on reusing training dataset poses serious privacy risks of neural network pruning due to the potentially increased memorization of training samples. %


\begin{figure}[!t]
    \centering
    \begin{subfigure}[b]{0.8\linewidth}
    \includegraphics[width=\linewidth]{figs/exp/cifar10_mobilenetv2_org.png}
    \caption{Original Model}
    \end{subfigure}
    \begin{subfigure}[b]{0.8\linewidth}
    \includegraphics[width=\linewidth]{figs/exp/cifar10_mobilenetv2_prune.png}
    \caption{Pruned Model}
    \end{subfigure}
    \caption{{Histogram of prediction confidences of the ground-truth label on the CIFAR10 MobileNetv2 model.} We remove 70\% of the parameters in the original model using l1 unstructured pruning. The figure shows the frequency of prediction confidences belonging to the ground-truth labels on the training and test data. The vertical lines indicate the average values of prediction confidence of training data (members) and test data (non-members). Neural network pruning makes the distance between two vertical lines larger than that in the original model, which indicates the increased divergence between prediction confidences over members and non-members after pruning.}
    \label{fig:histogram}
\end{figure}


Recent research has shown the privacy risks of neural networks, which are prone to memorizing sensitive information from the training data. Taking membership inference attack as an example, an adversary can infer whether a given data sample was used to train a neural network with high accuracy, which poses severe privacy threats of individual information.
For instance, if an adversary can infer that an individual's information is used to train a machine learning model for classifying the type of lung cancers, then the adversary knows that the individual has lung cancer.
Shorki \etal first conducted membership inference attacks by against black-box machine learning models, where the adversary only has access to the data sample and predictions of the target model.
Recently, membership inference attacks have been extended to a wide range of scenarios such as against white-box machine learning models~\cite{nasr2019comprehensive,leino2020stolen}, against generative models~\cite{hayes2019logan,chen2020gan} and graph models~\cite{olatunji2101membership}, against machine translation~\cite{hisamoto2020membership}, text generation systems~\cite{song2019auditing}, against genomic data~\cite{chen2020differential} and clinic data~\cite{jordon2020hide}, and against transfer learning models~\cite{zou2020privacy}.
Although extensive studies have investigated the privacy risks of neural networks, privacy leakage in pruned neural networks has not been investigated. 




In view of this, this paper focuses on one fundamental question: {\textit{comparing with deep neural networks, are the pruned networks more vulnerable to membership inference attacks?}}
Compared with conventional neural network training, neural network pruning may raise the privacy risks due to two main reasons: 
First, most neural network pruning approaches require re-training the pruned models on the training data for fine-tuning the parameters after removing the redundant parameters. 
The additional training process increases the risk of memorizing the sensitive training samples in the neural networks. 
Second, neural network pruning may disproportionately affect the predictions over training data and test/unseen data.
Although the model's overall prediction accuracy is not degraded due to pruning, the distribution of prediction confidences may be changed significantly. 
Figure~\ref{fig:histogram} shows the increased divergence between prediction confidences over training data (members) and test data (non-members) before and after pruning. 
Most existing membership inference attacks rely on the difference of predictions between members and non-members to predict the membership status. 
Given the increased divergence in neural network pruning, we hypothesize that the pruned models become more vulnerable to membership inference attacks.
Moreover, we observe that the such divergence varies among different classes or subgroups, which may provide more ``evidence'' for membership inference attacks and impose more serious threats.





Our main contributions are summarized below:
\vspace{-0.7em}
\begin{itemize}[leftmargin=*]
\item We conduct a pioneering study to explore the privacy risks of neural network pruning by performing membership inference attacks against the pruned models. 
To the best of our knowledge, this is the first work to analyze the privacy risks of neural network pruning. With the rising use of neural network pruning in end devices, we believe its privacy risks deserve more attention from the research community.
\vspace{-0.7em}
\item We propose two types of membership inference attacks specific to neural network pruning, namely class dependent membership inference attack (CDMIA) and self-attention-based membership inference attack (SAMIA). By analyzing the divergence of prediction confidences over members and non-members in the pruned models, both attacks result in high attack accuracy of identifying the membership status from the pruned models. Especially, the proposed SAMIA shows superiority in identifying the privacy risks of the pruned models by conducting a finer-grained analysis on the prediction confidences, which can be considered as a strong baseline attack for future research.
\vspace{-0.7em}
\item To rigorously evaluate the privacy risks of neural network pruning, we conduct extensive experiments of membership inference attacks on five commonly used datasets, four pruning approaches, seven sparsity levels, and 154 pruned models in total. From the experimental results, we demonstrate that neural network pruning indeed becomes more vulnerable to membership inference attacks. 
The adversary can successfully reveal the membership status, even without the knowledge of the pruning approach used in the target model. Moreover, we evaluate the privacy impacts of different pruning approaches and various sparsity levels.  
\vspace{-0.7em}
\item The existing defenses proposed for the unpruned models may become ineffective in mitigating the privacy risks due to neural network pruning. We propose a new defense approach, namely pair-based posterior balancing (PPB). PPB narrows the divergences of different prediction confidences during model fine-tuning based on their KL-divergence distance.
Our evaluation demonstrates that the proposed defense successfully mitigates the privacy risks due to neural network pruning compared with the original model while maintaining the pruned models' sparsity and prediction accuracy. 
\end{itemize}



==> change.tex <==
\large
\onecolumn
\setcounter{page}{1}

\begin{center}
\textbf{\Large Summary of Changes}
\end{center}
\vspace{2em}

\noindent Dear Reviewers, 
\vspace{1em}

\noindent The authors thank the reviewers for the careful reviews and constructive criticisms. We have carefully revised our manuscript according to the comments. For ease of review, we first quote the requested changes for this major revision below: 

\begin{enumerate}
\item Evaluate more realistic threat models, in particular scenarios where the adversary does not know the sparsity level or whether the victim's model is pruned or not.
\item Analysis with other existing attacks (e.g., NDSS'19, NDSS'21, and CSF'17) and defenses, especially DP, MemGuard, and/or transfer learning for the defenses.
\item Consider more datasets (i.e., Purchase-50, MNIST, and CH-MNIST), neural network architectures, and experimental setups (e.g., unevenly split datasets).
\item Include more in-depth analysis on the attack performance, (ideally, with some hypotheses and more experimental evaluation) in particular: (i) In what cases (model architectures, sparification method, sparsity level) does sparisification lead to increased privacy leakage, and why? (ii) How does the attack performance degrade as the adversary's sparsity level increasingly differs from the victim's? (iii) On the failure modes of self-attention; when it is expected to perform better or worse.
\item Figures 7 and 11 are quite dense and could benefit from splitting the results among several subplots, each targeted at a particular message.
\item Explain how pruning information is used in SAMIA (like what you did in the rebuttal but maybe with a new graph).
\end{enumerate}

We believe that the revised manuscript has been improved considerably and all the issues have been well resolved. The comments have been incorporated in the revised manuscript and additional comments are provided in this note. The review comments of the reviewers are copied below and the authors' corresponding responses to the comments from the reviewers are interspersed with the \textbf{Response} keyword. The major changes in the revised manuscript are highlighted in blue font.
\vspace{2em}

\noindent Sincerely,

\vspace{0.5em}
\noindent The authors




\newpage 
\begin{center}
\noindent {\Large\bf Response to the Requested Changes}
\end{center}

\noindent
\textbf{Comment 1:} \textit{Evaluate more realistic threat models, in particular scenarios where the adversary does not know the sparsity level or whether the victim's model is pruned or not.}

\vspace{1em}
\noindent
\textbf{Response 1:} Thank you for this comment. In the revised manuscript, we evaluate the privacy risk of the pruned neural network by considering the following three realistic threat models. 
\begin{itemize} \setlength{\itemsep}{0.1em} \setlength{\parskip}{0.1em}
\item Threat Model 1: The adversary knows the pruning approach and the sparsity level used in the pruned model. 
\item Threat Model 2: The adversary knows the pruning approach but not the sparsity level, where the target model might not be pruned, \ie, sparsity level $=0$.
\item Threat Model 3: The adversary has no knowledge of the pruning approach and sparsity level. 
\end{itemize}

Specifically, based on Threat Model 1, we evaluate the attack accuracy with different pruning approaches, sparsity levels, and target models and datasets. As shown in the revised Figure~\ref{fig:mia_cifar10_resnet},~\ref{fig:mia_cifar10_dense}~\ref{fig:mia_location}, we observe that the significant increase of privacy risks due to the neural network pruning. For ease of review, we quote the three figures below. More evaluation results can be found in Section~\ref{app:attack_acc} from the Appendix. 

\setcounter{figure}{6}
\begin{figure*}[!h]
\centering
\begin{subfigure}[b]{0.24\linewidth}
\includegraphics[width=0.95\linewidth]{figs/exp/mia/mia_cifar10_resnet18_level.pdf}
\caption{L1 unstructured}
\end{subfigure}
\begin{subfigure}[b]{0.24\linewidth}
\includegraphics[width=0.95\linewidth]{figs/exp/mia/mia_cifar10_resnet18_l1filter.pdf}
\caption{L1 structured}
\end{subfigure}
\begin{subfigure}[b]{0.24\linewidth}
\includegraphics[width=0.95\linewidth]{figs/exp/mia/mia_cifar10_resnet18_l2filter.pdf}
\caption{L2 structured}
\end{subfigure}
\begin{subfigure}[b]{0.24\linewidth}
\includegraphics[width=0.95\linewidth]{figs/exp/mia/mia_cifar10_resnet18_slim.pdf}
\caption{Slimming}
\end{subfigure}
\caption{Attack accuracy with different pruning approaches and sparsity levels (CIFAR10, ResNet18). The black line presents the attack accuracy of original models using Conf attack, \ie, Conf (Org.).}
\end{figure*}

\setcounter{figure}{7}
\begin{figure*}[!h]
\centering
\begin{subfigure}[b]{0.24\linewidth}
\includegraphics[width=0.95\linewidth]{figs/exp/mia/mia_cifar10_densenet121_level.pdf}
\caption{L1 unstructured}
\end{subfigure}
\begin{subfigure}[b]{0.24\linewidth}
\includegraphics[width=0.95\linewidth]{figs/exp/mia/mia_cifar10_densenet121_l1filter.pdf}
\caption{L1 structured}
\end{subfigure}
\begin{subfigure}[b]{0.24\linewidth}
\includegraphics[width=0.95\linewidth]{figs/exp/mia/mia_cifar10_densenet121_l2filter.pdf}
\caption{L2 structured}
\end{subfigure}
\begin{subfigure}[b]{0.24\linewidth}
\includegraphics[width=0.95\linewidth]{figs/exp/mia/mia_cifar10_densenet121_slim.pdf}
\caption{Slimming}
\end{subfigure}
\vspace{-0.5em}
\caption{Attack accuracy with different pruning approaches and sparsity levels (CIFAR10, DenseNet121).}
\end{figure*}

\setcounter{figure}{8}
\begin{figure}[H]
\centering
\includegraphics[width=0.24\linewidth]{figs/exp/mia/mia_location_column_level.pdf}
\caption{Attack accuracy with L1 unstructured pruning (Location, FC).}
\end{figure}

Based on Threat Model 2, the target model and the shadow model may use different sparsity levels in pruning. We evaluate the attack accuracy with unknown sparsity levels, where the cases that the target model or the shadow model is not pruned, \ie, sparsity level $=0$, are also considered. As shown in Figure~\ref{fig:unknown_sparsity_cifar10_dense},~\ref{fig:unknown_sparsity_location_fc}, the attack accuracy is not affected too much due to the different sparsity levels between target models and shadow models. In some cases, using a different sparsity level in pruning shadow models can increase the attack accuracy. The attack accuracy mainly depends on the performance of the shadow model, and thus the adversary can attack victim models with all sparsity levels with higher attack accuracy by selecting a good pruned shadow model. For instance, the adversary can use each shadow model to attack other shadow models with different sparsity levels and select the one with the highest attack accuracy. For ease of review, we quote the revision in Section~\ref{section:unknownSLPA} and Figure~\ref{fig:unknown_sparsity_cifar10_dense},~\ref{fig:unknown_sparsity_location_fc} below. More evaluation results can be found in the Appendix from Section~\ref{app:attack_unknown}.  

\vspace{0.5em}

\begin{displayquote}
\textbf{Unknown sparsity level.} We assume the adversary only knows the pruning approach but not the sparsity level that is the major factor of model efficiency. We evaluate the attack accuracy of SAMIA when the adversary prunes target models and shadow models using different sparsity levels. We also consider the case when the target model is not pruned, \ie, sparsity level $= 0$. As shown in Figure~\ref{fig:unknown_sparsity_cifar10_dense} and~\ref{fig:unknown_sparsity_location_fc}, the attack accuracy is not affected too much due to the different sparsity levels between target models and shadow models. In some cases, using a different sparsity level in pruning shadow models can increase the attack accuracy. The attack accuracy mainly depends on the performance of the shadow model. Thus the adversary can attack victim models with higher attack accuracy by selecting a good pruned shadow model. For instance, the adversary can use each shadow model to attack other shadow models with different sparsity levels and select the one with the highest attack accuracy.
\end{displayquote}


\setcounter{figure}{12}
\begin{figure*}[!h]
    \centering
    \begin{subfigure}[b]{0.24\linewidth}
    \includegraphics[width=\linewidth]{figs/exp/unknown/unknown_cifar10_densenet121_level.pdf}
    \caption{L1 Unstructured}
    \end{subfigure}
    \begin{subfigure}[b]{0.24\linewidth}
    \includegraphics[width=\linewidth]{figs/exp/unknown/unknown_cifar10_densenet121_l1filter.pdf}
    \caption{L1 Structured}
    \end{subfigure}
    \begin{subfigure}[b]{0.24\linewidth}
    \includegraphics[width=\linewidth]{figs/exp/unknown/unknown_cifar10_densenet121_l2filter.pdf}
    \caption{L2 Structured}
    \end{subfigure}
    \begin{subfigure}[b]{0.24\linewidth}
    \includegraphics[width=\linewidth]{figs/exp/unknown/unknown_cifar10_densenet121_slim.pdf}
    \caption{Slimming}
    \end{subfigure}
    \caption{Attack accuracy with unknown sparsity levels (CIFAR10, DenseNet121).}
\end{figure*}

\setcounter{figure}{13}
\begin{figure*}[!h]
\centering
\includegraphics[width=0.24\linewidth]{figs/exp/unknown/unknown_location_column_level.pdf}
\caption{Attack accuracy with unknown sparsity levels (Location, FC).}
\end{figure*}

Based on Threat Model 3, we conduct the experiments when the target model and the shadow model use different pruning approaches and sparsity levels in pruning. We conduct 20 experiments for each dataset and model and calculate the average attack accuracy loss. As shown in Table~\ref{tab:acc_loss_unknown}, we observe that without knowing both the sparsity levels and pruning approaches, the attack becomes ineffective in some scenarios (\eg, CIFAR10 VGG16 and CIFAR100 ResNet18), but can still successfully leak membership information in most cases. For ease of review, we quote the revision in Section~\ref{section:unknownSLPA} and Table~\ref{tab:acc_loss_unknown} below.


\begin{displayquote}
\textbf{Unknown sparsity level and pruning approach.} 
We assume the adversary has no prior knowledge of the sparsity level and pruning approach, where the adversary randomly picks a sparsity level and a pruning approach to prune the shadow model to attack the target pruned model. To evaluate the attack accuracy, we conduct 20 experiments for the aforementioned four image datasets and the corresponding neural networks. In each experiment, we randomly select the sparsity levels and pruning approaches for target models and shadow models, respectively, for example, target model using L1 Structured pruning with 0.5 sparsity level while shadow model using Slimming pruning with 0.8 sparsity level. 
The sparsity levels are selected from the set of $\{0.5, 0.6, 0.7, 0.8, 0.9\}$ and the pruning approaches are selected from the four pruning approaches.
To measure the privacy risks in the new threat model, we define the attack accuracy loss as $(acc_{known} - acc_{unknown}) /acc_{known}$, where $acc_{known}$ denotes the attack accuracy when the adversary knows all the pruning information and $acc_{unknown}$ denotes the attack accuracy without knowing any pruning information. 
Table~\ref{tab:acc_loss_unknown} shows the average attack accuracy loss over 20 experiments. We observe that without knowing both the sparsity levels and pruning approaches, the attack becomes ineffective in some scenarios (\eg, CIFAR10 VGG16 and CIFAR100 ResNet18), but can still successfully leak membership information in most cases.
\end{displayquote}
%

\setcounter{table}{0}
\begin{table}[!h]
\centering
\small
\begin{tabular}{@{}llr@{}}
\toprule
Dataset                                      & Model       & Attack Acc Loss \\ \midrule
\multirow{3}{*}{CIFAR10} & ResNet18    & 4.77\%          \\
                         & DenseNet121 & 1.63\%          \\
                         & VGG16       & 26.83\%         \\\hline
\multirow{3}{*}{CIFAR100}                    & ResNet18    & 12.41\%         \\
                                             & DenseNet121 & 6.90\%          \\
                                             & VGG16       & 2.43\%          \\\hline
\multirow{3}{*}{SVHN}                        & ResNet18    & 0.60\%          \\
                                             & DenseNet121 & 0.12\%          \\
                                             & VGG16       & 0.05\%          \\\hline
\multirow{3}{*}{CHMNIST}                     & ResNet18    & 0.78\%          \\
                                             & DenseNet121 & 0.52\%          \\
                                             & VGG16       & -0.58\%         \\ \bottomrule 
\end{tabular}%
\caption{Attack accuracy loss with unknown sparsity levels and pruning approaches.}
\vspace{-1em}
\end{table}

\newpage 
\noindent
\textbf{Comment 2:} \textit{Analysis with other existing attacks (e.g., NDSS'19, NDSS'21, and CSF'17) and defenses, especially DP, MemGuard, and/or transfer learning for the defenses.}

\vspace{1em}
\noindent
\textbf{Response 2:} Thank you for this comment. In the revised manuscript, to thoroughly evaluate the proposed attack, we consider eight existing MIAs, including the three attacks suggested by the reviewers and five other attacks, as well as three existing defenses.
\vspace{0.5em}

Specifically, for existing attacks, we first quote the description of the eight MIAs from Section 5.1.4.  


\begin{displayquote}
\begin{itemize}[leftmargin=*]\setlength{\itemsep}{0.1em} \setlength{\parskip}{0.1em}
    \item \textit{Ground-truth class confidence-based threshold attack (Conf)}. Yeom \etal used the prediction confidence of ground-truth class to identify membership status~\cite{yeom2018privacy}. The adversary learns a threshold to determine the membership of a data sample based on the confidence of ground-truth class. Given an input sample $\bm{x}$, its class $y$, and the pruned model $f_p$, the attack function is defined as $I_{\mathrm{conf}}(f_p, (\bm{x},y)) = \mathbbm{1}\{f_p^{(y)}(\bm{x})\geq\zeta_y\}$, where $f_p^{(y)}$ is the prediction confidence of class $y$ and $\zeta_y$ is the threshold of class $y$ derived from the shadow pruned model.
    \item \textit{Cross-Entropy-based threshold attack (Xent)}. The entropy loss can be used to derive the threshold from the shadow pruned model~\cite{yeom2018privacy}. The attack function is defined as $I_{\mathrm{xent}}(f_p, (\bm{x},y)) = \mathbbm{1}\{\mathrm{xent}(f_p^{(y)}(\bm{x}))\geq\zeta_y\}$, where $\mathrm{xent}$ denotes the cross entropy loss.
    \item \textit{Modified-entropy-based threshold attack (Mentr)}. Song and Mittal proposed modified entropy by including the information about the ground-truth class, which achieved better performance than using prediction confidence~\cite{song2020systematic}. The attack function is defined as $I_{\mathrm{mentr}}(f_p, (\bm{x},y)) = \mathbbm{1}\{\mathrm{mentr}(f_p^{(y)}(\bm{x}))\geq\zeta_y\}$, where $\mathrm{mentr}(f_p(\bm{x}), y) = - (1 - f_p^{(y)}(\bm{x}))\log (f_p^{(y)}(\bm{x})) - \sum_{t\neq y}f_p^{(t)}(\bm{x})\log(1-f_p^{(t)}(\bm{x}))$.
    \item \textit{Top1 Confidence-based threshold attack (Top1-Conf)}. Salem~\etal proposed to derive the threshold from the highest prediction confidence~\cite{salem2019ml}. The attack function is defined as $I_{\mathrm{top1}}(f_p, (\bm{x})) = \mathbbm{1}\{\mathrm{top1}(f_p(\bm{x}))\geq\zeta_y\}$, where $\mathrm{top1}$ calculates the highest value from the prediction confidence.
    \item \textit{Confidence-based Neural Network attack (NN)}. Shokri \etal proposed to use prediction confidence as features to train a neural network from the shadow model~\cite{shokri2017membership}, which is used to distinguish member and non-member data.
    \item \textit{Top-3 Confidence-based Neural Network attack (Top3-NN)}. Salem~\etal proposed to use the top-3 prediction confidences as features~\cite{salem2019ml} to train a neural network classifier.
    \item \textit{Confidence-based Neural Network attack with ground-truth class (NNCls)}. Nasr~\etal combined one-hot encoded class labels with the prediction confidence as features to train a neural network classifier~\cite{nasr2018machine}.
    \item \textit{Blind Membership Inference Attack (BlindMI)}. Hui~\etal proposed to determine the membership of a data sample by moving it to a non-member set and check if the moving operation increases the distance between member and non-member sets~\cite{huipractical}. BlindMI considers the data sample as a non-member if the distance is increased. We use the default BlindMI attack provided in~\cite{huipractical}.\vspace{-0.5em}
\end{itemize}
\end{displayquote}

In the main paper, we report the results of the four existing attacks that achieve the best attack accuracy in the pruned models, and the remaining results are presented in the Appendix. It should be mentioned that the proposed Class-Dependent MIA (CDMIA) in our previous manuscript is moved to the evaluation part as one of our basedline attack to better evaluate the performance of the proposed SAMIA. More details are discussed in the second point of Section: other major changes in the revision, at the end of this response letter. In general, by comparing the proposed SAMIA with the existing attacks, we observe SAMIA has advantages in identifying membership status in pruned models. The revised attack accuracy performance in Figure~\ref{fig:mia_cifar10_resnet},~\ref{fig:mia_cifar10_dense}~\ref{fig:mia_location} are quoted in Response 1. 
In addition, we further evaluate the impact of four key factors, \ie, prediction accuracy, confidence gap, sensitivity gap, and generalization gap presented in Section 4.1, on the attack performance. For ease of review, we quote the revised manuscript in Section 5.2.1 below. Figure~\ref{fig:acc_attack_cifar10_resnet},~\ref{fig:acc_attack_cifar10_densenet}, and~\ref{fig:acc_attack_location_fc} are quoted in Response 4 below. 


\begin{displayquote}
{\textbf{Impact of prediction accuracy, confidence gap, sensitivity gap, and generalization gap.}}
This section investigates the impacts of the above four key factors that may lead to the increase of privacy risks in the pruned models.
From Figure~\ref{fig:acc_attack_cifar10_resnet},~\ref{fig:acc_attack_cifar10_densenet}, and~\ref{fig:acc_attack_location_fc}, we observe that the attack accuracy is increased with the increase of \textit{prediction accuracy}. In addition, as aforementioned, we hypothesize that the increased \textit{confidence gap} and \textit{sensitivity gap} in neural network pruning can lead to increased membership inference risks. Meanwhile, overtraining is considered as one of the key causes of membership leakage in previous research~\cite{yeom2018privacy,song2020systematic}, leading to our evaluation on \textit{generalization gap}, \ie, the difference between training accuracy and testing accuracy. As shown in Figure~\ref{fig:gap_attack_cifar10_resnet18} and~\ref{fig:gap_attack_location_fc}, \textit{neural network pruning increases the gaps between members and non-members, \ie, confidence gap, sensitivity gap, and generalization gap, in most settings. Further, with the increase of gaps, we observe the increase of attack accuracy, which indicates the strong correlation between the gaps (confidence gap, sensitivity gap, and generalization gap) and the increased privacy risk.}
\end{displayquote}






\vspace{0.5em}
For defenses, the revised manuscript considers three existing defenses: 1) Basic Defense using Early Stopping and L2 Regularization~\cite{shokri2017membership,salem2019ml,song2020systematic}, 2) Differential Privacy~\cite{dwork2008differential}, 3) Adversarial Regularization~\cite{nasr2018machine}. Since the above three defenses can be implemented in the training/fine-tuning phase, which does not affect the efficiency of model prediction in the inference phase, we focus on these defenses. The MemGaurd is not considered in this revision, since MemGaurd needs to generate noise during the inference phase, which may not be feasible for resource-constraint devices using neural network pruning. For ease of review, we first quote the considered state-of-the-art defense description from Section 6.2.1 below. 

\vspace{0.5em}

\begin{displayquote}
\noindent
\textbf{Early Stopping and L2 Regularization (Basic).} 
Early stopping and l2 regularization have been used to successfully defend membership inference attacks with competitive performance~\cite{shokri2017membership,salem2019ml,song2020systematic}. As discussed in Section~\ref{4.1}, an adversary infers the membership of a sample based on the divergence of the prediction confidences between members and non-members. Such divergence becomes more severe as the number of training epochs increases, due to the increased memorization. Hence, the early stopping mechanism with fewer training epochs and l2 regularization for penalizing the over-training can tradeoff a slight reduction in model accuracy with lower privacy risk. 
In the evaluation, We stop the training and fine-tuning when the validation loss is not decreased for five epochs using early stopping mechanism. In l2 regularization, we set the regularization factor as $0.0005$. \textit{Note that we use early stopping and l2 regularization in all the other defenses to improve the defense performance.}

\noindent
\textbf{Differential Privacy (DP).}
Differential privacy is a strategy to bound the individual information exposure when running an algorithm $f$ and has been widely investigated for preventing privacy leakage against membership inference attacks~\cite{truex2019effects,rahimian2019differential,chen2020differential}.
In this paper, we use $(\epsilon, \delta)$-differential privacy to measure the privacy leakage. 
An algorithm $f$ is $(\epsilon, \delta)$-differential private on a dataset $\mathcal{D}$ if $\Pr(f(\mathcal{D})\in S) \leq \delta + e^{\epsilon}\Pr(f(\mathcal{D}') \in S),$
for any set $S$ of possible outputs of $f$ and neighbor dataset $D'$.
We apply the differentially private SGD algorithm (DP-SGD)~\cite{abadi2016deep} in the pruning process and investigate different privacy budgets $(\epsilon, \delta)$ by adding different Gaussian noises $\mathcal{N}(0, \sigma)$.

\noindent
\textbf{Adversarial Regularization (ADV).} 
Nasr~\etal proposed to consider the membership inference adversary in the training process~\cite{nasr2018machine}. The defender first trains a surrogate attack model to distinguish between members and non-members and then trains the target model to minimize the prediction loss while maximizing the classification loss of the surrogate attack model. A parameter $\alpha$ is used to balance the prediction performance and privacy risk. We apply Adversarial Regularization in the fine-tuning process of pruning.
\end{displayquote}
 

Upon the above defenses, the revised defense evaluation in Section 6.2.2 is quoted below.


\begin{displayquote}
Based on the settings of attack evaluations in Section~\ref{sec:eval}, we conduct the following experiments with defenses in the process of pruning. 
Since there is always a trade-off between privacy and prediction accuracy when implementing defenses, we explore different settings of hyper-parameters in the defensive mechanisms to thoroughly evaluate the defense performance. Specifically, we set hyper-parameter $\lambda \in \{1, 2,4,8, 16\}$ in PPB, $\sigma \in \{0.01, 0.1, 1, 10, 100\}$) in the DP noise vectors, $\alpha \in \{0.5, 1, 2, 4, 8, 16\}$ in ADV, respectively. 

Figure~\ref{fig:defense_cifar10_resnet_0.6} and Figure~\ref{fig:defense_location_0.6} respectively illustrate the prediction accuracy and attack accuracy with different defense mechanisms. For better illustration, we remove the results if the model with a specific hyper-parameter cannot achieve 75\% of the basic defense's prediction accuracy, \ie, poor prediction performance, or result in a higher attack accuracy, \ie, ineffective defense. We observe that PPB is especially effective in protecting all pruning approaches from attacks, which can reduce the attack accuracy to around 50\% (random guessing accuracy), while not degrading the prediction accuracy too much.
Hence, \textit{PPB defense can provide a privacy-preserving approach with minimal degradation of prediction accuracy}. 
In addition, ADV is also effective in the L1 unstructured and Slimming pruning, but fails to achieve a good balance between prediction performance and privacy in the L1 structured and L2 structured pruning. Similar to the fact shown in recent work~\cite{jayaraman2019evaluating}, we observe DP can hardly balance this utility-privacy tradeoff.
\end{displayquote}

\setcounter{figure}{15}
\begin{figure*}[!ht]
\centering
\begin{subfigure}[b]{0.24\textwidth}
\includegraphics[width=\linewidth]{figs/exp/defense/defend_cifar10_resnet18_level_0.6.pdf}
\caption{L1 Unstructured}
\end{subfigure}
\begin{subfigure}[b]{0.24\textwidth}
\includegraphics[width=\linewidth]{figs/exp/defense/defend_cifar10_resnet18_l1filter_0.6.pdf}
\caption{L1 Structured}
\end{subfigure}
\begin{subfigure}[b]{0.24\textwidth}
\includegraphics[width=\linewidth]{figs/exp/defense/defend_cifar10_resnet18_l2filter_0.6.pdf}
\caption{L2 Structured}
\end{subfigure}
\begin{subfigure}[b]{0.24\textwidth}
\includegraphics[width=\linewidth]{figs/exp/defense/defend_cifar10_resnet18_slim_0.6.pdf}
\caption{Slimming}
\end{subfigure}%
\caption{Performance of defenses (CIFAR10, ResNet18, Sparsity 0.6).}
\end{figure*}

\setcounter{figure}{17}
\begin{figure}[H]
\centering
\begin{subfigure}[b]{0.24\linewidth}\centering
\includegraphics[width=\linewidth]{figs/exp/defense/defend_location_column_level_0.6.pdf}
\caption{Defense against non-adaptive attacks}
\end{subfigure}
\begin{subfigure}[b]{0.24\linewidth}\centering
\includegraphics[width=\linewidth]{figs/exp/defense/defend_location_column_level_0.6_adp.pdf}
\caption{Defense against adaptive attacks}
\end{subfigure}
\vspace{-0.5em}
\caption{Performance of defenses (Location, FC, L1 Unstructured, Sparsity 0.6).}
\vspace{-0.5em}
\end{figure}


\newpage 
\noindent
\textbf{Comment 3:} \textit{Consider more datasets (i.e., Purchase-50, MNIST, and CH-MNIST), neural network architectures, and experimental setups (e.g., unevenly split datasets).}

\vspace{1em}
\noindent
\textbf{Response 3:} Thank you for this comment. In the revised manuscript, we include seven datasets which are commonly used in the membership inference evaluation, including two new datasets: Purchase and CH-MNIST dataset. 
We also investigated four widely-used neural network architecture: ResNet18, VGG16, DenseNet121, and Fully Connected Network. The results of the CIFAR10 and Purchase datasets are presented in the main paper and the rest of the results is included in the Appendix. For ease of review, we first quote the two new datasets from Section 5.1.1 below.


\vspace{0.5em}

\begin{displayquote}
\textit{CHMNIST}~\cite{kather2016multi}. This dataset consists of 5,000 histological images of human colorectal cancer containing 10 classes of tissues. We resize all images to $32\times 32$, the same dimension as CIFAR10 and CIFAR100.

\textit{Purchase}~\cite{acquire2014}. This dataset is presented in Acquire Valued Shoppers Challenge to predict which shoppers will become repeat buyers based on the purchase history. We use the preprocessed purchase dataset provided by Shokri \etal~\cite{shokri2017membership}, which contains 197,324 data samples, 600 binary features, and 100 classes. 
\end{displayquote}
\vspace{0.5em}

We investigated the experimental setups, where the datasets are unevenly split (Section~\ref{sec:dataset_split} in Appendix). Specifically, we split datasets into training, test, and validation using different ratios and evaluate the attack performance against the ResNet18 model on the CIFAR10 dataset.  As shown in Table~\ref{tab:split}, the unevenly split may cause a slight decrease of attack performance compared with evenly split, but the privacy risk is still high (over 70\% attack AUC). The revision from Section~\ref{sec:dataset_split} in Appendix is quoted below for the ease of review.

\vspace{0.5em}

\begin{displayquote}
This section reports the attack performance when the target model is trained on an unevenly split dataset. 
In the main paper, we split datasets into training, test, and validation in the ratio 45\%, 45\%, 10\%, so that we get the same number of training and test data and the random guessing attack accuracy is 50\%. Here we evaluate the attack performance using different and uneven ratios. Given the uneven dataset, we use Area Under the Curve (AUC) to report the attack performance. As shown in Table~\ref{tab:split}, the uneven split may cause a slight decrease of attack AUC compared with even split, but the privacy risk is still high (over 70\% attack AUC).
\setcounter{table}{1}
\begin{table*}[!h]
\centering
\begin{tabular}{@{}cc@{}}
\toprule
Dataset Split Ratio              & \multirow{2}{*}{Attack AUC} \\
Train(\%)/Test(\%)/Dev(\%) &                      \\ \midrule
45/45/10                  & 75.5                 \\
50/40/10                   & 72.7                 \\
60/30/10                   & 71.6                 \\ 
70/20/10                & 72.7 \\\bottomrule
\end{tabular}%
\caption{Impact of different dataset split strategies (CIFAR10, ResNet18, L1 Unstructured, Sparsity 0.7).}
\end{table*}
\end{displayquote}
%

\newpage 
\noindent
\textbf{Comment 4:} \textit{Include more in-depth analysis on the attack performance, (ideally, with some hypotheses and more experimental evaluation) in particular: (i) In what cases (model architectures, sparification method, sparsity level) does sparisification lead to increased privacy leakage, and why? (ii) How does the attack performance degrade as the adversary's sparsity level increasingly differs from the victim's? (iii) On the failure modes of self-attention; when it is expected to perform better or worse.}

\setcounter{figure}{9}
\begin{figure*}[!h]
    \centering
    \begin{subfigure}[b]{0.24\textwidth}
    \includegraphics[width=\linewidth]{figs/exp/impact/acc_attack_cifar10_resnet18.pdf}
    \caption{Prediction accuracy}
    \end{subfigure}
    \begin{subfigure}[b]{0.24\textwidth}
    \includegraphics[width=\linewidth]{figs/exp/impact/conf_gap_cifar10_resnet18.pdf}
    \caption{Confidence gap}
    \end{subfigure}
    \begin{subfigure}[b]{0.24\textwidth}
    \includegraphics[width=\linewidth]{figs/exp/impact/sens_gap_cifar10_resnet18.pdf}
    \caption{Sensitivity gap}
    \end{subfigure}
    \begin{subfigure}[b]{0.24\textwidth}
    \includegraphics[width=\linewidth]{figs/exp/impact/acc_gap_cifar10_resnet18.pdf}
    \caption{Generalization gap}
    \end{subfigure}
    \vspace{-0.5em}
    \caption{Impact of prediction accuracy, confidence gap, sensitivity gap, and generalization gap (CIFAR10, ResNet18).}
\end{figure*}

\begin{figure*}[!h]
    \centering
    \begin{subfigure}[b]{0.24\textwidth}
    \includegraphics[width=\linewidth]{figs/exp/impact/acc_attack_cifar10_densenet121.pdf}
    \caption{Prediction accuracy}
    \end{subfigure}
    \begin{subfigure}[b]{0.24\textwidth}
    \includegraphics[width=\linewidth]{figs/exp/impact/conf_gap_cifar10_densenet121.pdf}
    \caption{Confidence gap}
    \end{subfigure}
    \begin{subfigure}[b]{0.24\textwidth}
    \includegraphics[width=\linewidth]{figs/exp/impact/sens_gap_cifar10_densenet121.pdf}
    \caption{Sensitivity gap}
    \end{subfigure}
    \begin{subfigure}[b]{0.24\textwidth}
    \includegraphics[width=\linewidth]{figs/exp/impact/acc_gap_cifar10_densenet121.pdf}
    \caption{Generalization gap}
    \end{subfigure}
    \vspace{-0.5em}
    \caption{Impact of prediction accuracy, confidence gap, sensitivity gap, and generalization gap (CIFAR10, DenseNet121).}
\end{figure*}
\begin{figure*}[!h]
    \centering
    \begin{subfigure}[b]{0.24\textwidth}
    \includegraphics[width=\linewidth]{figs/exp/impact/acc_attack_location_column.pdf}
    \caption{Prediction accuracy}
    \end{subfigure}
    \begin{subfigure}[b]{0.24\textwidth}
    \includegraphics[width=\linewidth]{figs/exp/impact/conf_gap_location_column.pdf}
    \caption{Confidence gap}
    \end{subfigure}
    \begin{subfigure}[b]{0.24\textwidth}
    \includegraphics[width=\linewidth]{figs/exp/impact/sens_gap_location_column.pdf}
    \caption{Sensitivity gap}
    \end{subfigure}
    \begin{subfigure}[b]{0.24\textwidth}
    \includegraphics[width=\linewidth]{figs/exp/impact/acc_gap_location_column.pdf}
    \caption{Generalization gap}
    \end{subfigure}
    \vspace{-0.5em}
    \caption{Impact of prediction accuracy, confidence gap, sensitivity gap, and generalization gap (Location, FC).}
    \vspace{-1em}
\end{figure*}

\setcounter{figure}{0}
\begin{figure}[!h]
    \centering
    \begin{subfigure}[b]{0.48\linewidth}
    \centering
    \includegraphics[width=0.5\linewidth]{figs/mia_cifar10_densenet121_level_big_conf.pdf}
    \caption{Original model confidence}
    \end{subfigure}
    \begin{subfigure}[b]{0.48\linewidth}
    \centering
    \includegraphics[width=0.5\linewidth]{figs/mia_cifar10_densenet121_level_big_sens.pdf}
    \caption{Original model sensitivity}
    \end{subfigure}
    \begin{subfigure}[b]{0.48\linewidth}
    \centering
    \includegraphics[width=0.5\linewidth]{figs/mia_cifar10_densenet121_level_small_conf.pdf}
    \caption{Pruned model confidence}
    \end{subfigure}
    \begin{subfigure}[b]{0.48\linewidth}
    \centering
    \includegraphics[width=0.5\linewidth]{figs/mia_cifar10_densenet121_level_small_sens.pdf}
    \caption{Pruned model sensitivity}
    \end{subfigure}%
    \caption{Histograms of the prediction confidences and the prediction sensitivity of the ground-truth label on CIFAR10 and DenseNet121 model, respectively. We remove 70\% of the parameters in the original DenseNet121 model using l1 unstructured pruning on CIFAR10 dataset. The figures show the frequency of prediction confidence (a) and (c) and prediction sensitivity (b) and (d) belonging to the ground-truth class on the training and test data. The vertical lines indicate the average values of training data, \ie, members (black), and test data, \ie, non-members (red), respectively. In both prediction confidence and sensitivity measurements, neural network pruning makes the distances between the two vertical lines in the pruned model larger than that in the original model, which indicates a larger confidence gap and sensitivity gap between members and non-members due to pruning.}
\end{figure}


\vspace{1em}
\noindent
\textbf{Response 4:} Thank you for this comment. In this revised manuscript, we conduct in-depth analysis on the attack performance. The key revisions are listed as follows.

\vspace{0.5em}
(1) We investigate the impacts of four key factors that may lead to the increase of privacy risks in the pruned models. First, we observe that the attack accuracy is increased with the increase of \textit{prediction accuracy}, as shown in Figure~\ref{fig:acc_attack_cifar10_resnet},~\ref{fig:acc_attack_cifar10_densenet}, and~\ref{fig:acc_attack_location_fc}. Second, we propose two new metrics for pruned network privacy: \textit{prediction confidence} and \textit{prediction sensitivity}. Specifically, given an input sample $\bm{x}$ and an pruned model $f_p$, the prediction confidence is defined as $\mathrm{PC} = f_p(\bm{x})$. 
Prediction sensitivity measures the prediction behavior changes in terms of slight input change, which is defined as
\begin{equation}
    \mathrm{PS} = \frac{1}{n} \sum_i^n  \frac{|f_p(\bm{x} + \epsilon\bm{\delta_i}) - f_p(\bm{x})|}{\epsilon},\vspace{-0.5em}
\end{equation}
where $\bm{\delta_i} \sim \mathcal{N}(0, 1), i\in\{1,2, \cdots, n\}$ is a random Gaussian noise vector added to the input data $\bm{x}$, and  $\epsilon$ controls the magnitude of input changes. We observe the increased divergence between members and non-members in terms of prediction confidence and prediction sensitivity (Figure~\ref{fig:histogram}). Therefore, we hypothesize that the increased \textit{confidence gap} and \textit{sensitivity gap} in neural network pruning can lead to increased membership inference risks.
Third, overtraining is considered as one of the key causes of membership leakage in previous research~\cite{yeom2018privacy,song2020systematic}, leading to our evaluation on \textit{generalization gap}, \ie, the difference between training accuracy and testing accuracy. As shown in Figure~\ref{fig:gap_attack_cifar10_resnet18},~\ref{fig:gap_attack_cifar10_densenet121}, and~\ref{fig:gap_attack_location_fc}, \textit{neural network pruning increases the gaps between members and non-members, \ie, confidence gap, sensitivity gap, and generalization gap, in most settings. Further, with the increase of gaps, we observe the increase of attack accuracy, which indicates the strong correlation between the gaps (confidence gap, sensitivity gap, and generalization gap) and the increased privacy risk.} The revision from Section~\ref{sec:5.2.1} is quoted below for the ease of review.



\vspace{0.5em}

\begin{displayquote}
\textbf{Impact of prediction accuracy, confidence gap, sensitivity gap, and generalization gap.}
This section investigates the impacts of the above four key factors that may lead to the increase of privacy risks in the pruned models.
From Figure~\ref{fig:acc_attack_cifar10_resnet},~\ref{fig:acc_attack_cifar10_densenet}, and~\ref{fig:acc_attack_location_fc}, we observe that the attack accuracy is increased with the increase of \textit{prediction accuracy}. In addition, as aforementioned, we hypothesize that the increased \textit{confidence gap} and \textit{sensitivity gap} in neural network pruning can lead to increased membership inference risks. Meanwhile, overtraining is considered as one of the key causes of membership leakage in previous research~\cite{yeom2018privacy,song2020systematic}, leading to our evaluation on \textit{generalization gap}, \ie, the difference between training accuracy and testing accuracy. As shown in Figure~\ref{fig:gap_attack_cifar10_resnet18} and~\ref{fig:gap_attack_location_fc}, \textit{neural network pruning increases the gaps between members and non-members, \ie, confidence gap, sensitivity gap, and generalization gap, in most settings. Further, with the increase of gaps, we observe the increase of attack accuracy, which indicates the strong correlation between the gaps (confidence gap, sensitivity gap, and generalization gap) and the increased privacy risk.}
\end{displayquote}


Furthermore, we investigate the impact of different pruning methods. We observe that different pruning approaches result in different prediction accuracy at a certain sparsity level. Thus, we consider both the attack accuracy and prediction accuracy in investigating the privacy risks of different pruning approaches. The attack accuracy of most pruning approaches can be higher than that of the original models, given the similar prediction accuracy, which indicates the exaggerated privacy risks due to neural network pruning. The revision is quoted below.

\vspace{0.5em}

\begin{displayquote}
\textbf{Impact of pruning approaches.}
This section investigates the impact of different pruning approaches. As shown in Figure~\ref{fig:prune_acc}, different pruning approaches result in different prediction accuracy at a certain sparsity level. Thus, we consider both the attack accuracy and prediction accuracy in investigating the privacy risks of different pruning approaches. 
As shown in Figure~\ref{fig:acc_attack_cifar10_resnet},~\ref{fig:acc_attack_cifar10_densenet}, and~\ref{fig:acc_attack_location_fc}, given the similar prediction accuracy of the pruned models, L1 unstructured and slimming pruning result in the highest attack accuracy. 
\textit{The attack accuracy of most pruning approaches can be higher than that of the original models, given the similar prediction accuracy, } which indicates the exaggerated privacy risks due to neural network pruning.
\end{displayquote}
\vspace{0.5em}

(ii) We conduct evaluation to investigate the attack performance, when the adversary's sparsity levels are different from the victim's. As shown in Figure~\ref{fig:unknown_sparsity_cifar10_dense} and~\ref{fig:unknown_sparsity_location_fc}, the attack accuracy is not affected too much due to the different sparsity levels between target models and shadow models. In some cases, using a different sparsity level in pruning shadow models can increase the attack accuracy. The attack accuracy mainly depends on the performance of shadow model, and thus the adversary can attack victim models with all sparsity levels with higher attack accuracy by selecting a good pruned shadow model. For instance, the adversary can use each shadow model to attack other shadow models with different sparsity levels and select the one with the highest attack accuracy. The revision is quoted below for the ease of review.

\vspace{0.5em}

\begin{displayquote}
\textbf{Unknown sparsity level.} We assume the adversary only knows the pruning approach but not the sparsity level that is the major factor of model efficiency. We evaluate the attack accuracy of SAMIA when the adversary prunes target models and shadow models using different sparsity levels. We also consider the case when the target model is not pruned, \ie, sparsity level $= 0$. As shown in Figure~\ref{fig:unknown_sparsity_cifar10_dense} and~\ref{fig:unknown_sparsity_location_fc} (Comment 1), the attack accuracy is not affected too much due to the different sparsity levels between target models and shadow models. In some cases, using a different sparsity level in pruning shadow models can increase the attack accuracy. The attack accuracy mainly depends on the performance of shadow model, and thus the adversary can attack victim models with higher attack accuracy by selecting a good pruned shadow model. For instance, the adversary can use each shadow model to attack other shadow models with different sparsity levels and select the one with the highest attack accuracy.
\end{displayquote}
\vspace{0.5em}

(iii) Our proposed SAMIA results in the highest attack accuracy than the existing MIAs in most experimental settings. We observe that SAMIA does not perform among the best attacks mainly in two scenarios: 1) the attack accuracy is close to 50\% (\ie, random guessing), \eg, Figure~\ref{fig:mia_svhn_resnet},~\ref{fig:mia_chmnist_vgg}. 2) the sparsity level is low (\eg, $0.5$). When the sparsity level is low, the divergence of confidence and sensitivity is reduced. Thus, the features of confidence and sensitivity cannot be fully utilized for SAMIA, which makes the SAMIA's attack performance close to the existing attacks. The revision is quoted below for the ease of revision.

\vspace{0.5em}

\begin{displayquote}
We observe that SAMIA does not perform among the best attacks mainly in two cases: 1) the attack accuracy is close to 50\% (\ie, random guessing), \eg, Figure~\ref{fig:mia_svhn_resnet},~\ref{fig:mia_chmnist_vgg}. 2) the sparsity level is low (\eg, $0.5$). When the sparsity level is low, the divergence of confidence and sensitivity is reduced. In this case, the features of confidence and sensitivity cannot be fully utilized for SAMIA, which makes the SAMIA's attack performance close to the existing attacks.
\end{displayquote}
%

\newpage 
\noindent
\textbf{Comment 5:} \textit{Figures 7 and 11 are quite dense and could benefit from splitting the results among several subplots, each targeted at a particular message.}

\vspace{1em}
\noindent
\textbf{Response 5:} Thank you for this comment. In the revised manuscript, we have split the figures into several subplots, each targeting at a single pruning approach. The revised figures are quoted below for the ease of review. More evaluation results can be found in Section~\ref{app:attack_acc} from the Appendix. 

\setcounter{figure}{6}
\begin{figure*}[!h]
\centering
\begin{subfigure}[b]{0.24\linewidth}
\includegraphics[width=0.95\linewidth]{figs/exp/mia/mia_cifar10_resnet18_level.pdf}
\caption{L1 unstructured}
\end{subfigure}
\begin{subfigure}[b]{0.24\linewidth}
\includegraphics[width=0.95\linewidth]{figs/exp/mia/mia_cifar10_resnet18_l1filter.pdf}
\caption{L1 structured}
\end{subfigure}
\begin{subfigure}[b]{0.24\linewidth}
\includegraphics[width=0.95\linewidth]{figs/exp/mia/mia_cifar10_resnet18_l2filter.pdf}
\caption{L2 structured}
\end{subfigure}
\begin{subfigure}[b]{0.24\linewidth}
\includegraphics[width=0.95\linewidth]{figs/exp/mia/mia_cifar10_resnet18_slim.pdf}
\caption{Slimming}
\end{subfigure}
\caption{Attack accuracy with different pruning approaches and sparsity levels (CIFAR10, ResNet18). The black line presents the attack accuracy of original models using Conf attack, \ie, Conf (Org.).}
\end{figure*}

\setcounter{figure}{7}
\begin{figure*}[!h]
\centering
\begin{subfigure}[b]{0.24\linewidth}
\includegraphics[width=0.95\linewidth]{figs/exp/mia/mia_cifar10_densenet121_level.pdf}
\caption{L1 unstructured}
\end{subfigure}
\begin{subfigure}[b]{0.24\linewidth}
\includegraphics[width=0.95\linewidth]{figs/exp/mia/mia_cifar10_densenet121_l1filter.pdf}
\caption{L1 structured}
\end{subfigure}
\begin{subfigure}[b]{0.24\linewidth}
\includegraphics[width=0.95\linewidth]{figs/exp/mia/mia_cifar10_densenet121_l2filter.pdf}
\caption{L2 structured}
\end{subfigure}
\begin{subfigure}[b]{0.24\linewidth}
\includegraphics[width=0.95\linewidth]{figs/exp/mia/mia_cifar10_densenet121_slim.pdf}
\caption{Slimming}
\end{subfigure}
\vspace{-0.5em}
\caption{Attack accuracy with different pruning approaches and sparsity levels (CIFAR10, DenseNet121).}
\end{figure*}

\setcounter{figure}{8}
\begin{figure}[H]
\centering
\includegraphics[width=0.24\linewidth]{figs/exp/mia/mia_location_column_level.pdf}
\caption{Attack accuracy with L1 unstructured pruning (Location, FC).}
\end{figure}

\newpage 
\noindent
\textbf{Comment 6:} \textit{Explain how pruning information is used in SAMIA (like what you did in the rebuttal but maybe with a new graph).}

\vspace{1em}
\noindent
\textbf{Response 6:} Thank you for this comment. In the revised manuscript, we have improved the description of SAMIA in the paper. Morevoer, given the newly identified sensitivity metric in pruned models, we have updated the attack model by including the sensitivity as part of the input features. We have also added more attention heads in the attack model to capture different representations among feature spaces. The multi-head self-attention has become one of the driving forces behind recent advances in NLP models. The description of SAMIA and the new figure are quoted below.


\begin{displayquote}
Upon the above observations, we propose one hypothesis: \textit{the divergences among classes, \ie, confidence gap and sensitivity gap, can provide fine-grained ``evidence'' for MIAs, leading to serious privacy leakage}. In addition, most existing MIA research only considers the confidence gap and a single threshold of the ground-truth class, which may under-estimates the privacy risks of MIAs in neural network pruning. Hence, we propose SAMIA, a self-attention MIA, to fully utilize the increased divergence information along with the class information to conduct a finer-grained analysis.

In SAMIA, we leverage the self-attention mechanism to automatically extract the finer-grained ``thresholds'' from different classes by capturing the dependency between predicted information (confidence and sensitivity) and class information and allowing them to interact with each other. Specifically, SAMIA takes the pruned model's prediction confidence and sensitivity and ground-truth labels as inputs.  Given a specific class, the self-attention mechanism finds out the specific confidence information and sensitivity information that the attack ``threshold'' should pay more ``attention'' to.
\end{displayquote}
 

\setcounter{figure}{4}
\begin{figure}[!h]
\centering
\includegraphics[width=0.3\linewidth]{figs/tranformer.pdf}
\caption{Attack model architecture in SAMIA.}
\end{figure}


\begin{displayquote}
Figure~\ref{fig:transformer} illustrates the network architecture of the attack model used in SAMIA, enlighten by the idea of Transformer~\cite{vaswani2017attention}, \ie, one of the most widely used self-attention architecture. We first convert the ground-truth label into a one-hot vector and then feed both the pruned model's prediction confidence and sensitivity and the one-hot vector into the attack model as the input features. 
The input features are encoded into a vector using a Fully Connected (FC) layer, which are then fed into the multi-head self-attention modules. In each module, we encode the features as query $Q$, key $K$, and value $V$ vectors using a linear function following the self-attention strategy.
\end{displayquote}



\begin{displayquote}
Compared with existing MIAs that learn a single threshold of prediction confidence to determine the membership, the proposed SAMIA captures the information of confidences and sensitivities and intuitively better learns the diverse thresholds to multiple classes. Our evaluation results demonstrate that SAMIA leads to higher attack accuracy compared with the state-of-the-art attacks.
\end{displayquote}


\newpage 
\noindent {\large\bf Other Major Changes in the Revision}

\vspace{1em}
\noindent \textbf{1. Introduce ``sensitivity gap" as a new privacy risk metric.} We identify a new attack vector in pruned models, \ie, prediction sensitivity, which is calculated as the change of output given slight input change (Eq.~\ref{eq:sensitivity}). We find that the sensitivity gap between members and non-members will be increased due to neural network pruning, which can be utilized by the adversary for membership inference attack. Figure~\ref{fig:sens_gap_cifar10_resnet},~\ref{fig:sens_gap_cifar10_dense}, and~\ref{fig:sens_gap_location} show the strong correlation between sensitivity gap and attack accuracy. More discussions can be found in the response to Comment 4.

\vspace{1em}
\noindent
\textbf{2. Move ``Class-Dependent MIA (CDMIA)'' to attack evaluation as one baseline attack.} In the previous manuscript, we describe the two class-dependent MIAs, \ie, CDMIA and SAMIA, against the pruned models in Section 4, ``Membership Inference Attacks against Neural Network Pruning''. Specifically, CDMIA is a threshold based attack using prediction confidence and modified entropy (\ie, Conf and Mentr in this manuscript). In the revised manuscript, we include other existing attacks against pruned models, \eg threshold-based attack (Xent, Top1-Conf), neural network-based attacks (NN, Top3-NN), and BlindMI attack.  
Hence, to clearly present the proposed SAMIA and thoroughly evaluate SAMIA, we move the description of CDMIA attacks to the evaluation section (Section~\ref{sec:state_mia}) as two of the eight state-of-the-art MIAs to evaluate the performance of SAMIA. 

\vspace{1em}
\noindent
\textbf{3. Explore the utility-privacy trade-off in defenses.}
In the previous submission, we select a hyper-parameter to report the effectiveness of our proposed PPB defense and the existing defenses. In this paper, we explore the utility-privacy trade-off in each defense by evaluating the defense performance using different hyper-parameters. We report the curve of prediction accuracy and attack accuracy for each setting and compare them among all the defenses. 

First, We find our proposed PPB can successfully reduce the confidence gap and sensitivity gap as shown in Figure~\ref{fig:hist_defense}. Furthermore, the reduced gaps can be preserved in different classes, as shown in Figure~\ref{fig:div_cls_defense}. The revision from Section~\ref{sec:defense_eval} is quoted as below.

\vspace{0.5em}
\begin{displayquote}
Figure~\ref{fig:hist_defense} demonstrates the effectiveness of the proposed PPB. By comparing Figure~\ref{fig:hist_defense} with Figure~\ref{fig:histogram}, we observe the divergence between member and non-member data is significantly reduced by applying PPB defense. 
Such decreased divergence can be observed in different classes (Comparing Figure~\ref{fig:cls_div} with Figure~\ref{fig:div_cls_defense} in Appendix). 
By changing the distributions of the pruned model's posterior predictions, the PPB defense makes the attack model fail to learn the binary classification thresholds from the prediction confidence and sensitivity.\end{displayquote}

\setcounter{figure}{14}
\begin{figure}[!h]
\centering
\begin{subfigure}[b]{0.24\linewidth}
\centering
\includegraphics[width=\linewidth]{figs/mia_cifar10_densenet121_level_small_conf_pair_2.pdf}
\caption{Confidence gap}
\end{subfigure}    
\begin{subfigure}[b]{0.24\linewidth}
\centering
\includegraphics[width=\linewidth]{figs/mia_cifar10_densenet121_level_small_sens_pair_2.pdf}
\caption{Sensitivity gap}
\end{subfigure}
\vspace{-0.5em}
\caption{Divergence of the pruned model's prediction confidences and sensitivities using PPB defense (CIFAR10, DenseNet121).} %
\vspace{-0.5em}
\end{figure}

\setcounter{figure}{18}
\begin{figure*}[!h]
\centering
\begin{subfigure}[b]{0.24\linewidth}
\centering
\includegraphics[width=\linewidth]{figs/conf_gap_cifar10_densenet121_level_pair2.pdf}
\caption{Confidence gap}
\end{subfigure}    
\begin{subfigure}[b]{0.24\linewidth}
\centering
\includegraphics[width=\linewidth]{figs/sens_gap_cifar10_densenet121_level_pair2.pdf}
\caption{Sensitivity gap}
\end{subfigure}
\caption{Divergence of the pruned model's prediction confidences and sensitivities over different classes with PPB defense (CIFAR10, DenseNet121). } 
\end{figure*}


Second, we demonstrate that PPB is especially effective in protecting all pruning approaches from attacks. In most experimental settings, PPB can reduce the attack accuracy to around 50\% (random guessing accuracy), while not degrading the prediction accuracy too much. ADV is also effective in the L1 unstructured and Slimming pruning, but fails to achieve a good balance between prediction performance and privacy in the L1 structured and L2 structured pruning. 
The settings of all defenses and key defense results are quoted below for the ease of review. 



\vspace{0.5em}

\begin{displayquote}
Based on the settings of attack evaluations in Section~\ref{sec:eval}, we conduct the following experiments with defenses in the process of pruning. 
Since there is always a trade-off between privacy and prediction accuracy when implementing defenses, we explore different settings of hyper-parameters in the defensive mechanisms to thoroughly evaluate the defense performance. Specifically, we set hyper-parameter $\lambda \in \{1, 2,4,8, 16\}$ in PPB, $\sigma \in \{0.01, 0.1, 1, 10, 100\}$) in the DP noise vectors, $\alpha \in \{0.5, 1, 2, 4, 8, 16\}$ in ADV, respectively. 
\end{displayquote}


\setcounter{figure}{15}
\begin{figure*}[!h]
\centering
\begin{subfigure}[b]{0.24\textwidth}
\includegraphics[width=\linewidth]{figs/exp/defense/defend_cifar10_resnet18_level_0.6.pdf}
\caption{L1 Unstructured}
\end{subfigure}
\begin{subfigure}[b]{0.24\textwidth}
\includegraphics[width=\linewidth]{figs/exp/defense/defend_cifar10_resnet18_l1filter_0.6.pdf}
\caption{L1 Structured}
\end{subfigure}
\begin{subfigure}[b]{0.24\textwidth}
\includegraphics[width=\linewidth]{figs/exp/defense/defend_cifar10_resnet18_l2filter_0.6.pdf}
\caption{L2 Structured}
\end{subfigure}
\begin{subfigure}[b]{0.24\textwidth}
\includegraphics[width=\linewidth]{figs/exp/defense/defend_cifar10_resnet18_slim_0.6.pdf}
\caption{Slimming}
\end{subfigure}%
\caption{Performance of defenses (CIFAR10, ResNet18, Sparsity 0.6).}
\end{figure*}

\begin{figure*}[!h]
\centering
\begin{subfigure}[b]{0.24\textwidth}
\includegraphics[width=\linewidth]{figs/exp/defense/defend_cifar10_resnet18_level_0.6_adp.pdf}
\caption{L1 Unstructured}
\end{subfigure}
\begin{subfigure}[b]{0.24\textwidth}
\includegraphics[width=\linewidth]{figs/exp/defense/defend_cifar10_resnet18_l1filter_0.6_adp.pdf}
\caption{L1 Structured}
\end{subfigure}
\begin{subfigure}[b]{0.24\textwidth}
\includegraphics[width=\linewidth]{figs/exp/defense/defend_cifar10_resnet18_l2filter_0.6_adp.pdf}
\caption{L2 Structured}
\end{subfigure}
\begin{subfigure}[b]{0.24\textwidth}
\includegraphics[width=\linewidth]{figs/exp/defense/defend_cifar10_resnet18_slim_0.6_adp.pdf}
\caption{Slimming}
\end{subfigure}%
\caption{Performance of defenses against adaptive attacks (CIFAR10, ResNet18, Sparsity 0.6).}
\vspace{-0.5em}
\end{figure*}

\begin{figure}[!h]
\centering
\begin{subfigure}[b]{0.24\linewidth}\centering
\includegraphics[width=\linewidth]{figs/exp/defense/defend_location_column_level_0.6.pdf}
\caption{Defense against non-adaptive attacks}
\end{subfigure}
\begin{subfigure}[b]{0.24\linewidth}\centering
\includegraphics[width=\linewidth]{figs/exp/defense/defend_location_column_level_0.6_adp.pdf}
\caption{Defense against adaptive attacks}
\end{subfigure}
\vspace{-0.5em}
\caption{Performance of defenses (Location, FC, L1 Unstructured, Sparsity 0.6).}
\vspace{-0.5em}
\end{figure}

\vspace{0.5em}

\begin{displayquote}
Figure~\ref{fig:defense_cifar10_resnet_0.6} and Figure~\ref{fig:defense_location_0.6} respectively illustrate the prediction accuracy and attack accuracy with different defense mechanisms. For better illustration, we remove the results if the model with a specific hyper-parameter cannot achieve 75\% of the basic defense's prediction accuracy, \ie, poor prediction performance, or result in a higher attack accuracy, \ie, ineffective defense. We observe that PPB is especially effective in protecting all pruning approaches from attacks, which can reduce the attack accuracy to around 50\% (random guessing accuracy), while not degrading the prediction accuracy too much.
Hence, \textit{PPB defense can provide a privacy-preserving approach with minimal degradation of prediction accuracy}. 
In addition, ADV is also effective in the L1 unstructured and Slimming pruning, but fails to achieve a good balance between prediction performance and privacy in the L1 structured and L2 structured pruning. Similar to the fact shown in recent work~\cite{jayaraman2019evaluating}, we observe DP can hardly balance this utility-privacy tradeoff.
\end{displayquote}

\vspace{1em}

Third, we investigate the defense performance against adaptive attacks. we find PPB can reduce the accuracy of adaptive attacks compared to the attacks on the pruned model without defenses, which mitigates the privacy threats. PPB and ADV are the best two defenses for the L1 unstructured and Slimming pruning. PPB also provides the best protection in L1 structured and L2 structured pruning. The revision is quoted below.

\vspace{0.5em}

\begin{displayquote}
As shown in Figure~\ref{fig:defense_cifar10_resnet_0.6_adp} and~\ref{fig:defense_location_0.6_adp}, we observe that \textit{PPB can reduce the accuracy of adaptive attacks compared to the attacks on the pruned model without defenses}, which mitigates the privacy threats.
Besides, PPB and ADV are the best two defenses for the L1 unstructured and Slimming pruning. PPB provides the best protection in L1 structured and L2 structured pruning. 
\end{displayquote}


==> response.tex <==
\large
\onecolumn
\setcounter{page}{1}

\begin{center}
\textbf{\Large Summary of Changes}
\end{center}
\vspace{2em}
\noindent \textbf{Paper Title}: Membership Inference Attacks and Defenses in Neural Network Pruning

\vspace{0.5em}
\noindent \textbf{Submission ID}: USENIX Security '22 Fall \#444

\vspace{3em}
\noindent Dear Reviewers, 

\vspace{1em}
\noindent The authors would like to gratefully thank the reviewers for their valuable comments and suggestions that help to improve this work. We have carefully revised our manuscript according to the revision plan and the reviewers' comments, beginning with the major suggestions from the shepherd (Comment 1-3) and followed by the major comments from the reviewers (Comment 4-12).

\vspace{0.5em}
\noindent For ease of review, the major changes in the revised manuscript are highlighted in blue font and quoted below. Thanks again to the reviewers for their suggestions.

\vspace{1em}
\noindent Warm Regards,

\vspace{0.5em}
\noindent The Authors

\vspace{3em}
\par\noindent
\textbf{Comment 1:} Some reviewers are not satisfied with additional datasets only being used in the attack evaluation. It is expected that this weakness is addressed by either significantly removing the defense claim or evaluating the defense using new datasets. (Reviewer A and E) 

\vspace{0.5em}
\par\noindent
\textbf{Response:}
Due to the space limit, in the previous manuscript, the defense evaluation on the new datasets was discussed in the Appendix. The evaluation results from the new datasets are consistent with those from the previous datasets. In the revised manuscript, we have included the new datasets and defense results in the main paper, including Figure 7, 8, 10, 11, 13, 17, 19, and the corresponding analysis in Section 5 and Section 6. The rest of the experimental results will be provided in a public extended version. The link is included in the paper (we blind the link for anonymity in the submission).

\vspace{2em}
\par\noindent\textbf{Comment 2:} A few reviewers are not satisfied with your comparison/evaluation with DP. You should either make a proper claim or evaluate DP in the experiment. (Reviewer A and E)

\vspace{0.5em}\par\noindent
\textbf{Response:}
We implemented differential privacy (DP) defense using differentially private SGD (DPSGD), which is one of the most widely-used defense techniques to train neural networks with DP guarantees~\cite{abadi2016deep,rahimian2019differential}. Specifically, based on DPSGD, we first clip the gradient, then add noise to the gradient, and use the generated noisy gradient to update the model’s parameters. The noise is sampled from a Gaussian distribution $\mathcal{N}(0,\sigma)$. To achieve ($\epsilon, \delta$)-DP in DPSGD, the standard deviation of the Gaussian distribution, i.e., $\delta$, should be in the order of $\Omega(q\sqrt{T\log (1/\delta)/\epsilon}$, where $q$ denotes the sampling ratio, and $T$ denotes the total number of iterations. Accordingly, the privacy guarantee of the DP defense can be derived from $\delta$. Additionally, $\delta$ plays an important role in balancing utility and privacy. Thus, we explored the different values of $\delta$ in the defense evaluation. %

In the revised manuscript, we have discussed DP with the detailed experimental settings in Section 6.3.1 and compared the proposed defense with DP, which is quoted below for ease of review.

\vspace{0.5em}
Differential privacy is a strategy to bound the individual information exposure when running an algorithm $f$ and has been widely investigated for preventing privacy leakage against membership inference attacks~\cite{truex2019effects,rahimian2019differential,chen2020differential}.
We implement differentially private SGD (DPSGD)~\cite{abadi2016deep,rahimian2019differential}, one of the most widely-used defense techniques, to train neural networks with DP guarantees. 
Following DPSGD, we first clip the gradient, then add noise to the gradient, and use the generated noisy gradient to update the model's parameters. The noise is sampled from a Gaussian distribution $\mathcal{N}(0,\sigma)$. To achieve ($\epsilon, \delta$)-DP, the standard deviation of the Gaussian distribution, i.e., $\delta$, should be in the order of $\Omega(q\sqrt{T\log (1/\delta)/\epsilon}$, where $q$ denotes the sampling ratio and $T$ denotes the total number of iterations.
Accordingly, the privacy guarantee of the DP defense can be derived from $\delta$, which plays an important role in balancing utility and privacy.
Therefore, in the defense evaluation, we evaluate the effectiveness of DP defense and explore the impact of different privacy budgets (\ie, different values of $\delta$).




\vspace{2em}
\par\noindent
\textbf{Comment 3:} A few reviewers are worried that the revision is way too long with much information will be skipped in the 18-page camera ready. And the takeaway messages are often unclear. We hope that the authors can properly address this point. (Reviewer D)

\vspace{0.5em}\par\noindent
\textbf{Response:} In the revised manuscript, we have moved the major experimental results to the main paper. The rest of the experimental results will be provided in an extended version. Besides, we have substantially improved the experimental results to make the takeaway messages clear, detailed in Response to Comment 4 below.


\vspace{2em}
\par\noindent
\textbf{Comment 4:} In-depth Analysis of Experimental Results. (Reviewer A, D, E)
\vspace{0.5em}\par\noindent
\textbf{Response:} In the revised manuscript, we provide more in-depth discussion and takeaway messages of experimental results in Section 5.2. 

\begin{itemize}
\item We first investigated the privacy risks of neural network pruning in Section 5.2.1. The simulation results demonstrated the increased privacy risks of pruning. Detailed discussions are quoted below.

\vspace{0.5em}

Since different pruning approaches and sparsity levels may achieve distinct prediction accuracy, to make a fair comparison, we evaluate the privacy risks of pruning by taking the prediction accuracy into consideration. 
Figure~\ref{fig:acc_attack} show the relationship between prediction accuracy and (SAMIA) attack accuracy when we apply different pruning approaches and sparsity levels on the CIFAR10, CIFAR100, and Location datasets.
We observe that \textit{when the pruned model achieves a comparable prediction accuracy with the original model, most pruning approaches result in an increased attack accuracy (\ie, privacy risk).
}
The attack accuracy may be decreased with the loss of prediction accuracy, as the pruned model becomes less effective for both prediction and attack.
However, we still observe that in most cases, when the pruned model performs worse than the original model, the pruned model's attack accuracy remains higher than the original one's. 
Therefore, the pruned models become more vulnerable to membership inference attacks than the original models.

When a low sparsity level is used, we always observe the increased privacy risk of the pruned model (Figure~\ref{fig:mia_sparsity}). Since with a low sparsity level, the pruned model is more likely to achieve a comparable or even higher prediction accuracy compared with the original model, which increases the accuracy of prediction confidence used in MIAs and further increases the privacy risk.


\vspace{0.5em}
\item We then identified the correlation between increased privacy risk and the three gaps, \ie, confidence gap, sensitivity gap, and generalization gap in Section 5.2.2. The strong correlation between the gaps (confidence gap, sensitivity gap) and the increased privacy risk validates our intuition that the increased confidence and sensitivity gap may lead to higher privacy risks. Detailed discussions are quoted below.

\vspace{0.5em}

As aforementioned, we hypothesize that neural network pruning leads to the increased \textit{confidence gap} and \textit{sensitivity gap} (in ground-truth class) of pruned models, thus increasing their membership inference risks. 
Meanwhile, overtraining is considered as one of the key causes of membership leakage in previous research~\cite{yeom2018privacy,song2020systematic}, leading to our evaluation on \textit{generalization gap}, \ie, the difference between training accuracy and testing accuracy. 
From Figure~\ref{fig:gap_cifar10_resnet18}, we observe that {neural network pruning increases the gaps between members and non-members, \ie, confidence gap, sensitivity gap, and generalization gap, in most settings}. Further, with the increase of gaps, we observe the increase of attack accuracy, which indicates  \textit{the strong correlation between the gaps, \ie, confidence gap, sensitivity gap, and generalization gap, and the increased privacy risk.}

The strong correlation for confidence gap and sensitivity gap validates our intuition that these gaps can be leveraged by the adversary to infer the membership status, introducing a new attack surface in neural network pruning. 
By investigating the attack results, we find that the confidence gap plays the most important role in the privacy risk. L1 unstructured and slimming pruning usually lead to an increased confidence gap, which will be leveraged by the adversary and result in a higher attack accuracy. Additionally, sensitivity gap can also leak the membership information. For example, the confidence gap of L1 unstructured pruning on a CIFAR10 ResNet18 model (Figure~\ref{fig:conf_gap_cifar10_resnet18}) is close to the original model, but due to the increased sensitivity gap (Figure~\ref{fig:sens_gap_cifar10_resnet}), the pruning still results in an increased attack accuracy.


\vspace{0.5em}
\item Next, we investigated the privacy risks of different pruning approaches in Section 5.2.3. The reasons for their distinct privacy risks were discussed, which are quoted below. 

\vspace{0.5em}

Following the same settings above, we investigate the privacy risks of different pruning approaches by comparing the attack accuracy under the similar prediction accuracy.
As shown in Figure~\ref{fig:acc_attack} and~\ref{fig:mia_sparsity}, given the similar prediction accuracy of the pruned models, L1 unstructured and slimming pruning result in the highest attack accuracy. 
Besides, L1 structured pruning achieves the lowest attack accuracy among all pruning approaches, but still in some cases, the attack accuracy is higher than the original model, even with the similar or lower prediction accuracy.
The structured constraint used in L1 structured pruning regularizes the model in the fine-tuning and thereby reduces the privacy risk.


\vspace{0.5em}
\item Fourth, we discussed the effectiveness of the proposed SAMIA attack in Section 5.2.4, and quoted the discussion below. More discussions are also detailed in response to Comment 12. 

\vspace{0.5em}

To investigate the effectiveness of the proposed SAMIA, we compare SAMIA with the state-of-the-art MIAs in terms of attack accuracy. As shown in Figure~\ref{fig:mias_cifar10_resnet}, we observe that \textit{our proposed SAMIA achieves the highest attack accuracy in most cases compared with baseline attacks}, which is mainly due to the fact that SAMIA best leverages both confidence gap and sensitivity gap (in ground-truth class) introduced in pruning. Besides, Top1-conf and Mentr attacks are also effective, as both attacks take advantage of the confidence gap, the most important factor for model privacy. 
We also observe that when the pruning introduces a high generalization gap , all attacks can achieve a high attack accuracy (\eg, CIFAR100 DenseNet121 in Figure~\ref{fig:mias_cifar100_densenet1},~\ref{fig:mias_cifar100_densenet2} and Appendix Figure~\ref{fig:gen_gap_cifar100_densenet})), which has been discussed in the previous MIA research.


\vspace{0.5em}
\item Fifth, we analyzed the attack performance without the knowledge of sparsity levels and pruning approaches and investigated the cause of unsuccessful attacks in this setting in Section 5.2.5. The discussions are quoted below. 

\vspace{0.5em}

\textbf{Unknown sparsity level and pruning approach.} 

Since we assume the adversary has no prior knowledge of the sparsity level and pruning approach, the adversary may randomly pick a sparsity level and a pruning approach to prune a shadow model for attacks. To evaluate the attack accuracy, we conduct 20 experiments for the aforementioned four image datasets and the corresponding neural networks. In each experiment, we randomly select the sparsity levels and pruning approaches for target models and shadow models, respectively. For example, the target model uses L1 Structured pruning with 0.5 sparsity level while the shadow model uses Slimming pruning with 0.8 sparsity level. The sparsity levels are selected from the set of $\{0.5, 0.6, 0.7, 0.8, 0.9\}$ and the pruning approaches are selected from the four pruning approaches.
To measure the privacy risks, we define the attack accuracy loss as $(acc_{known} - acc_{unknown}) /acc_{known}$, where $acc_{known}$ denotes the attack accuracy when the adversary knows all the pruning information and $acc_{unknown}$ denotes the attack accuracy without knowing any pruning information. Table~\ref{tab:acc_loss_unknown} shows the average attack accuracy loss over 20 experiments for each dataset and model. 
We observe that \textit{without knowing the sparsity levels and pruning approaches, the attack is still effective in most cases except the CIFAR10 VGG16 and CIFAR100 ResNet18 models}.
The poor attack performance in these two models is due to the ineffectiveness of shadow models using specific sparsity levels and pruning approaches for attacks.
For example, we observe a significant drop of attack accuracy (from 90\% to 50\%) when applying L1 structured and slimming pruning with sparsity levels 0.7 to 0.9, on the CIFAR10 VGG16 model (Figure~\ref{fig:mia_cifar10_vgg16} in Appendix). The large gap makes the shadow models pruned using these settings ineffective in attacking the unknown victim model. 


\vspace{0.5em}
\item Further, we explained the reason for experimental variation in the experimental results in Section 5.1.5, which is quoted below.

\vspace{0.5em}

Due to the large number of settings evaluated in the attacks and defenses and the high computational cost in each setting, we conduct all the experiments only once. Thus experimental variation may be observed due to the randomness in neural network pruning and membership inference attacks (\eg, parameter initialization, dataset shuffling).
\end{itemize}

\vspace{2em}
\par\noindent
\textbf{Comment 5:} Acknowledge lack of privacy guarantee. (Reviewer A)

\vspace{0.5em}\par\noindent\textbf{Response:} The proposed PPB defense is only verified in the empirical experiments, which has been acknowledged in Section 6.3.2 of the revised manuscript.

\vspace{0.5em}
The defenses are evaluated by the empirical experiments. We will investigate the strict privacy guarantee in future work.



\vspace{2em}
\par\noindent\textbf{Comment 6:} Discussion of label-only membership inference attack. (Reviewer B and E)
\vspace{0.5em}\par\noindent\textbf{Response:} 
This paper did not consider label-only membership inference attacks because they require a different assumption about the adversary's capability – the adversary only knows the output class rather than the probability. We agree that it is realistic that the pruned model is under the attack of the label-only setting. To address the issue of unknown prediction probability, our proposed attack could be integrated with the existing label-only attacks that use data augmentation and black-box adversarial attacks~\cite{choquette2021label,li2021membership}. One possible challenge might be the effectiveness of black-box adversarial attacks, since the moderate model sparsity may help prevent the adversarial attacks~\cite{xiao2018training}. 
In the revised manuscript, label-only membership inference attacks has been discussed as one future direction in Section 7, which is quoted below for ease of review.

\vspace{0.5em}

The proposed SAMIA attack will be further explored under more challenging MIA settings, such as the label-only MIA without available confidences, where the existing label-only MIA attacks using data augmentation~\cite{choquette2021label} and black-box adversary~\cite{li2021membership} can be potentially integrated for more powerful attack capability. 



\vspace{2em}
\par\noindent\textbf{Comment 7:} How to find and tune the neural network architecture. (Reviewer D)
\vspace{0.5em}\par\noindent\textbf{Response:} We chose the typical victim model and attack model architectures, and optimization approach that are widely used in the existing membership inference work~\cite{shokri2017membership,hui2019practical,salem2019ml,song2020systematic}. In the revised manuscript, we have clarified the experimental settings, including how to choose datasets, neural network architectures, and optimization approaches. This manuscript does not consider the tuning of the neural network architecture. The revision in Section 5.1 is quoted below for ease of review.

\vspace{0.5em}

In the evaluation, we consider the most widely used datasets, neural network architectures, and optimization approaches following recent research of MIAs~\cite{shokri2017membership,hui2019practical,salem2019ml,song2020systematic}.



\vspace{2em}
\par\noindent\textbf{Comment 8:} Difficulty of generating noise on resource-constrained devices. (Reviewer E)
\vspace{0.5em}\par\noindent
\textbf{Response:} In this work, we consider the defenses that generate noise in the training phase, e.g., differentially private SGD (DPSGD) and adversarial regularization (ADV). Because the purpose of pruning techniques is to reduce the computational cost in the inference phase, it might not be feasible to generate carefully crafted noises during inference, which incurs additional costs. Hence, we did not consider MemGuard, which generates adversarial examples for misleading the adversary’s classifier in the inference phase. In the revised manuscript, we have clarified this in \textit{the second point} of the design principle of defenses in Section 6.1, which is quoted below for ease of review.

\vspace{0.5em}

\par\noindent
\textbf{Design Principles of Defenses}


Two major design principles are considered for the defenses of pruned neural networks. On the one hand, effective defenses should be able to reduce the behavior discrepancy introduced by pruning. The above attack evaluation has demonstrated that the privacy risks introduced by MIAs in the pruned models is due to the increased divergence of prediction confidences and sensitivities. Hence, it is essential to reduce such divergence between members and non-members of the pruned neural networks for defense. On the other hand, the defenses need to take into consideration the resource constraints imposed by low-end devices. Neural network pruning aims to reduce the computational cost during inference. 
Such cost cannot be increased by the defenses. Therefore, the defenses should be designed mitigate the privacy risks of pruned models before deploying them on devices, thus without introducing additional defense costs in the inference phase. 



\vspace{2em}
\par\noindent\textbf{Comment 9:} Improve editorial quality. (Reviewer D)
\vspace{0.5em}\par\noindent\textbf{Response:} We have made significant improvements to the writing.


\vspace{2em}
\par\noindent\textbf{Comment 10:} Release code. (Reviewer A)
\vspace{0.5em}\par\noindent
\textbf{Response:} We have included a link to the code (we blind the link for anonymity in the submission).


\vspace{2em}
\par\noindent\textbf{Comment 11:} PPB and ADV are the best two defenses for the L1 unstructured and Slimming pruning. -> Why? Again, I would hope to see a mode in-depth discussion. (Reviewer D) Section 6.2.3 does not describe what is the adaptive attack mounted on the shadow pruned model (which the attacker has full knowledge of, as described in the text). (Reviewer E)
\vspace{0.5em}\par\noindent
\textbf{Response:} 
In the revised manuscript, we have clarified the evaluation for defenses against adaptive attacks and provided a more detailed analysis of the experimental results in Section 6.3.3. The revision is quoted below for ease of review.

\vspace{0.5em}

In adaptive attacks, the adversary trains a shadow pruned model following the same defense mechanism (\eg, Basic, DP, ADV, and proposed PPB) and pruning process. The adversary then performs the SAMIA attack based on the shadow pruned model.


As shown in Figure~\ref{fig:defense_cifar10_resnet0.6_adp} and~\ref{fig:defense_l1unstructured_0.6_adp}, we observe that PPB reduces the accuracy of adaptive attacks compared to the attacks on the pruned model without defenses and provides the best protection in L1 structured and L2 structured pruning. Besides, for the L1 unstructured and Slimming pruning, PPB and ADV are the best two defenses. 
\textit{PPB is designed towards pruned models by reducing the confidence and sensitivity gap. Therefore, in general, PPB provides good protection in all pruning approaches.
}
In addition, ADV is designed to mitigate the confidence gap, which is largely increased in L1 unstructured and slimming pruning (as discussed in Section~\ref{sec:impact_gap}). Hence, ADV is also effective in protecting pruned models using L1 unstructured and slimming pruning.




\vspace{2em}
\par\noindent
\textbf{Comment 12:} The new evaluation suggests that SAMIA does not outperform Salem et al. in regimes where pruning does not affect prediction accuracy. What is the motivation for the newly introduced privacy sensitivity? Is it specific to SAMIA or does it also explain leakage from other attacks? Why does it explain membership leakage if the information it computes over is not used by the attack? (Reviewer E)
\vspace{0.5em}\par\noindent
\textbf{Response:} 
In the revised manuscript, we have discussed the effectiveness of SAMIA in Section 5.2.4 and the impact of sensitivity gap introduced in pruning in Section 5.2.2. 
The pruned neural network enforces a small number of parameters to achieve similar prediction capabilities with the original neural network, which increases the memorization of training data and makes the pruned model more sensitive to the training data. Hence, such increased memorization can intuitively lead to a larger divergence of the prediction confidences and sensitivities between members and non-members.
Figure~\ref{fig:histogram} confirms our intuition: the pruning leads to the increased confidence gap and sensitivity gap between members and non-members. Such gaps can be leveraged by the adversary to infer membership status. This motivates us to include both confidence and sensitivity in the SAMIA attack. Besides, the introduced privacy sensitivity is specific to SAMIA. 
As shown in Figure 11, 12, 13, and 14, SAMIA achieves the highest attack accuracy compared with baseline attacks in most cases. This is mainly due to the fact that SAMIA best leverages both confidence gap and sensitivity gap. By further investigating Figure 7(d), 8(d), 9(d), and 10(d), we find that when pruning introduces a high generalization gap, all attacks can achieve a high attack accuracy. The revision is quoted below for ease of review. 


\vspace{0.5em}

\noindent\textbf{Impact of confidence and sensitivity gap}

The strong correlation for confidence gap and sensitivity gap validates our intuition that these gaps can be leveraged by the adversary to infer the membership status, introducing a new attack surface in neural network pruning. 
By investigating the attack results, we find that the confidence gap plays the most important role in the privacy risk. L1 unstructured and slimming pruning usually lead to an increased confidence gap, which will be leveraged by the adversary and result in a higher attack accuracy. Additionally, sensitivity gap can also leak the membership information. For example, the confidence gap of L1 unstructured pruning on a CIFAR10 ResNet18 model (Figure~\ref{fig:conf_gap_cifar10_resnet18}) is close to the original model, but due to the increased sensitivity gap (Figure~\ref{fig:sens_gap_cifar10_resnet}), the pruning still results in an increased attack accuracy.

\vspace{0.5em}
\noindent\textbf{Effectiveness of SAMIA}

To investigate the effectiveness of the proposed SAMIA, we compare SAMIA with the state-of-the-art MIAs in terms of attack accuracy. As shown in Figure~\ref{fig:mias_cifar10_resnet}, we observe that \textit{our proposed SAMIA achieves the highest attack accuracy in most cases compared with baseline attacks}, which is mainly due to the fact that SAMIA best leverages both confidence gap and sensitivity gap (in ground-truth class) introduced in pruning. Besides, Top1-conf and Mentr attacks are also effective, as both attacks take advantage of the confidence gap, the most important factor for model privacy. 
We also observe that when the pruning introduces a high generalization gap , all attacks can achieve a high attack accuracy (\eg, CIFAR100 DenseNet121 in Figure~\ref{fig:mias_cifar100_densenet1},~\ref{fig:mias_cifar100_densenet2} and Appendix Figure~\ref{fig:gen_gap_cifar100_densenet})), which has been discussed in the previous MIA research.


